The Compound Information Bottleneck Outlook

We formulate and analyze the compound information bottleneck programming. In this problem, a Markov chain $ \mathsf{X} \rightarrow \mathsf{Y} \rightarrow \mathsf{Z} $ is assumed with fixed marginal distributions $\mathsf{P}_{\mathsf{X}}$ and $\mathsf{P}_{\mathsf{Y}}$, and the mutual information between $ \mathsf{X} $ and $ \mathsf{Z} $ is sought to be maximized over the choice of conditional probability of $\mathsf{Z}$ given $\mathsf{Y}$ from a given class, under the \textit{worst choice} of the joint probability of the pair $(\mathsf{X},\mathsf{Y})$ from a different class. We consider several classes based on extremes of: mutual information; minimal correlation; total variation; and the relative entropy class. We provide values, bounds, and various characterizations for specific instances of this problem: the binary symmetric case, the scalar Gaussian case, the vector Gaussian case and the symmetric modulo-additive case. Finally, for the general case, we propose a Blahut-Arimoto type of alternating iterations algorithm to find a consistent solution to this problem.

==> preamble/beamer_numbering_style.tex <==
\newtheorem{question}{Question}
\newtheorem{answer}{Answer}
\newtheorem{approach}{Approach}
%\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{observation}{Observation}
\newtheorem{suggestion}{Suggestion}
\newtheorem{conclusion}{Conclusion}
\newtheorem{idea}{Idea}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{goal}{Our Goal}
\newtheorem{conjecture}{Conjecture}


\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}

\newcommand{\mf}[1]{\mathfrak{#1}} % mathfrak 
\newcommand{\dd}{\mathop{}\!\text{d}} % For dx in integrals or derivatives

\newcommand{\aconj}[1]{#1^{(\mathfrak{a})}}
\newcommand{\bconj}[1]{#1^{(\mathsf{b})}}
\newcommand{\abconj}[1]{#1^{(\mathfrak{a\!b})}}
\newcommand{\ba}{r}
\newcommand{\bmap}{b^-_{a^+}}
\newcommand{\apam}{a^+_{a^-}}
\newcommand{\symm}[1]{\accentset{\textcolor{red}{\circ}}{#1}}
\newcommand{\properup}{\overset{p}{\succcurlyeq}}
\newcommand{\properde}{\overset{p}{\preccurlyeq}}
\newcommand{\upgradec}[1]{\check{#1}}

\DeclareMathOperator{\arctanh}{arctanh}

\DeclareMathOperator{\ext}{ext}
\DeclareMathOperator{\Lev}{Lev}
\DeclareMathOperator{\sgn}{sgn}

\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\tr}{tr}

\newcommand\hcancel[2][black]{\setbox0=\hbox{$#2$}%
	\rlap{\raisebox{.45\ht0}{\textcolor{#1}{\rule{\wd0}{1pt}}}}#2} 

==> preamble/beamer_specific.tex <==
\usepackage{multicol}


\definecolor{darkolivegreen}{rgb}{0.33, 0.42, 0.18}
\definecolor{olive}{rgb}{0.5, 0.5, 0.0}
\definecolor{sacramentostategreen}{rgb}{0.0, 0.34, 0.25}
\definecolor{pantone 200}{RGB}{186,12,47}
\definecolor{pantone 280}{RGB}{0,32,91}
\definecolor{frenchRed}{HTML}{EF4531}
\definecolor{frenchPink}{HTML}{f38eff}
\definecolor{frenchBlue}{HTML}{0055A4}
\definecolor{frenchGrey}{HTML}{dee1ec}
\definecolor{frenchLightBlue}{HTML}{becbff}
\definecolor{lightblue}{HTML}{a6cee3}
\definecolor{navyblue}{HTML}{1f78b4}
\definecolor{lightgreen}{HTML}{00adb5}
\definecolor{aussieBlue}{HTML}{00008B}
\definecolor{aussieRed}{HTML}{FF0000}
\definecolor{aussieWhite}{HTML}{FFFFFF}


\mode<presentation> {
	\useinnertheme{rounded}
	\useoutertheme{infolines}
	\usecolortheme{wolverine}
	\setbeamercovered{invisible}
	\usefonttheme[onlylarge]{structurebold}
}
\setbeamertemplate{headline}[default]
\setbeamertemplate{navigation symbols}{}
\setbeamertemplate{itemize items}[square] %Small triangles
\setbeamertemplate{enumerate items}[default] %Just numbers

\setbeamercolor{itemize item}{fg=frenchRed}

\setbeamercolor{block title}{fg=yellow!80!orange,bg=darkblue!80!black}
\setbeamercolor{block body}{fg=black,bg=blue!10!white}
\setbeamercolor{alerted text}{fg=frenchRed} 

\setbeamercolor{section in head/foot}{bg=blue!0!black,fg=white}

\setbeamerfont{footline}{size=\fontsize{6}{6}\selectfont}
\setbeamercolor{left in foot}{fg=white, bg=aussieBlue}
\setbeamercolor{center in foot}{fg=white, bg=aussieRed}
\setbeamercolor{right in foot}{fg=black, bg=aussieWhite}

\setbeamercolor{frametitle}{fg=yellow!80!orange,bg=frenchBlue}

\setbeamercolor{title}{fg=yellow!80!orange,bg=frenchBlue}

==> preamble/beamer_specific_isit2021.tex <==
\usepackage{multicol}


\definecolor{darkolivegreen}{rgb}{0.33, 0.42, 0.18}
\definecolor{olive}{rgb}{0.5, 0.5, 0.0}
\definecolor{sacramentostategreen}{rgb}{0.0, 0.34, 0.25}
\definecolor{pantone 200}{RGB}{186,12,47}
\definecolor{pantone 280}{RGB}{0,32,91}
\definecolor{frenchRed}{HTML}{EF4531}
\definecolor{frenchPink}{HTML}{f38eff}
\definecolor{frenchBlue}{HTML}{0055A4}
\definecolor{frenchGrey}{HTML}{dee1ec}
\definecolor{frenchLightBlue}{HTML}{becbff}
\definecolor{lightblue}{HTML}{a6cee3}
\definecolor{navyblue}{HTML}{1f78b4}
\definecolor{lightgreen}{HTML}{00adb5}
\definecolor{aussieBlue}{HTML}{00008B}
\definecolor{aussieRed}{HTML}{FF0000}
\definecolor{aussieWhite}{HTML}{f5f5f5}


\mode<presentation> {
	\useinnertheme{rounded}
	\useoutertheme{infolines}
	\usecolortheme{wolverine}
	\setbeamercovered{invisible}
	\usefonttheme[onlylarge]{structurebold}
}
\setbeamertemplate{headline}[default]
\setbeamertemplate{navigation symbols}{}
\setbeamertemplate{itemize items}[square] %Small triangles
\setbeamertemplate{enumerate items}[default] %Just numbers

\setbeamercolor{itemize item}{fg=frenchRed}

\setbeamercolor{block title}{fg=yellow!80!orange,bg=darkblue!80!black}
\setbeamercolor{block body}{fg=black,bg=blue!10!white}
\setbeamercolor{alerted text}{fg=frenchRed} 

\setbeamercolor{section in head/foot}{bg=blue!0!black,fg=white}

\setbeamerfont{footline}{size=\fontsize{6}{6}\selectfont}
\setbeamercolor{left in foot}{fg=white, bg=aussieBlue}
\setbeamercolor{center in foot}{fg=white, bg=aussieRed}
\setbeamercolor{right in foot}{fg=black, bg=aussieWhite}

\setbeamercolor{frametitle}{fg=yellow!80!orange,bg=frenchBlue}

\setbeamercolor{title}{fg=yellow!80!orange,bg=frenchBlue}

==> preamble/book_numbering_style.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[chapter]
%\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

%\theoremstyle{remark}
%\theoremstyle{proposition}
\newtheorem{remark}{Remark}

%\newtheorem*{remark}{Remark}

\newtheorem{lemma}{Lemma}
\newtheorem{conjecture}{Conjecture}


\newtheorem{example}{Example}

\newtheorem{question}{Question}
\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{\ \rule{0.5em}{0.5em}}


%\theoremstyle{proposition}
\newtheorem{proposition}{Proposition}[chapter]
\providecommand*\propositionautorefname{Proposition}
\renewcommand{\subsectionautorefname}{Subsection\negthinspace}

\providecommand*\lemmaautorefname{Lemma}



\newtheorem{claim}{Claim}
\newtheorem{notation}{Notation}[theorem]


==> preamble/glossary.tex <==
%\newglossaryentry{bs}{name=BS, description = {Base station}}

\newglossaryentry{dmic}{name={DM-IC},description={discrete memoryless interference channel}}

\newglossaryentry{dof}{name={DoF},description={degrees of freedom}}

\newglossaryentry{mu}{name=MU, description = {Mobile User}}



==> preamble/packages_beamer.tex <==
%\usepackage[latin1]{inputenc}
%\usepackage{amsmath}
%\usepackage{amsfonts}
%\usepackage{amssymb}


\usepackage{amsthm}
\usepackage{bbm}
%\usepackage{bm}
%\usepackage{cancel}
%\usepackage{ClearSans}
%\usepackage{cleveref}


%\usepackage{epsfig}

%\usepackage[T1]{fontenc}

\usepackage{glossaries}
%\usepackage[margin=1in]{geometry}
%\usepackage[dvips]{graphicx}





%\usepackage{IEEEtrantools}
%\usepackage{mathrsfs}
%\usepackage{mathtools}
\usepackage{pgfplots}

%\usepackage{scalerel}
%\usepackage[binary-units]{siunitx}


%
\usepackage{tikz}
%
%%\usepackage{upquote}
%
%
\usetikzlibrary{arrows,decorations.markings, shapes.arrows}
\usetikzlibrary{calc,intersections, positioning,graphs,fit}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{graphs}
\usetikzlibrary{overlay-beamer-styles}
\usetikzlibrary{decorations.text}










==> preamble/specific.tex <==
\tikzset{naming/.style={align=center,font=\small}}
\tikzset{antenna/.style={insert path={-- coordinate (ant#1) ++(0,0.25) -- +(135:0.25) + (0,0) -- +(45:0.25)}}}
\tikzset{station/.style={naming,draw,shape=dart,shape border rotate=90, minimum width=10mm, minimum height=10mm,outer sep=0pt,inner sep=3pt}}
%\tikzset{mobile/.style={naming,draw,shape=rectangle,minimum width=15mm,minimum height=7.5mm, outer sep=0pt,inner sep=3pt}}

\newcommand{\BS}[1]{%
	\begin{tikzpicture}
	\node[station] (base) {#1};
	
	%\draw[line join=bevel] (base.110) -- (base.70) -- (base.north west) -- (base.north east) -- cycle;
	\draw[line join=bevel] (base.100) -- (base.80) -- (base.110) -- (base.70) -- (base.north west) -- (base.north east);
	\draw[line join=bevel] (base.100) -- (base.70) (base.110) -- (base.north east);
	
	% original yshift=.8pt
	\draw[line cap=rect] ([yshift=0pt]base.north) [antenna=1];
	\end{tikzpicture}
}



==> sections/binary.tex <==
Here we consider the case where $ \rv{X} $, $ \rv{Y} $, and $ \rv{Z} $ are binary random variables. 

For a specific setup of uniform binary random variables, the channel from $ \rv{X} $ to $ \rv{Y} $ is completely defined for any $ \mathsf{P}_{\rv{Z}|\rv{Y}} $, as specified in the following theorem.
\begin{theorem}
	Suppose $ \rv{X} $ and $ \rv{Y} $ are $ \Ber(1/2) $ random variables. Then,  $ \mathsf{P}_{\rv{X}\rv{Y}} $ is a \acrfull{dsbs} with parameter $ \alpha $, i.e.,
	\begin{equation}
		\mathsf{P}_{\rv{X}\rv{Y}}(x,y) = \frac{1}{2} (\alpha \cdot \mathbbm{1}(x \neq y) + (1-\alpha)
		\mathbbm{1}(x=y)),
	\end{equation}
	where $ \alpha =  h_b^{-1} (1-C_1) $.
	Furthermore, the optimal $ \mathsf{P}_{\rv{Z}|\rv{Y}} $ is a \acrshort{bsc} with parameter $ \beta $, given by $ \beta =  h_b^{-1} (1-C_2) $. The oblivious rate is thus
	\begin{equation}
		R(C_1,C_2) = 1- h_b(\alpha * \beta),
	\end{equation}
	where $ * $ is the binary convolution.
\end{theorem}
\begin{proof}
	Probability marginalization yields the following system of equalities:
	\begin{align}
		\frac{1}{2} &= \Prob{\rv{Y}=1} = \Prob{\rv{Y}=1|\rv{X}= 0} \Prob{\rv{X}= 0} +\Prob{\rv{Y}=1|\rv{X}= 1} \Prob{\rv{X}= 1} \\
		&=\frac{1}{2} \left[ \Prob{\rv{Y}=1|\rv{X}= 0} + \Prob{\rv{Y}=1|\rv{X}= 1} \right],
	\end{align}
	and
	\begin{align}
		\frac{1}{2} &= \Prob{\rv{Y}=0} = \Prob{\rv{Y}=0|\rv{X}= 0} \Prob{\rv{X}= 0} +\Prob{\rv{Y}=0|\rv{X}= 1} \Prob{\rv{X}= 1} \\
		&=\frac{1}{2} \left[ \Prob{\rv{Y}=0|\rv{X}= 0} + \Prob{\rv{Y}=1|\rv{X}= 1} \right].
	\end{align}
	This implies that
	\begin{align}
		 \Prob{\rv{Y}=1|\rv{X}= 0} = 1- \Prob{\rv{Y}=1|\rv{X}= 1}  = \alpha = \Prob{\rv{Y}=0|\rv{X}= 1} = 1-\Prob{\rv{Y}=0|\rv{X}= 0}.
	\end{align}
	Considering the respective mutual information between random variables $ \rv{X} $ and $ \rv{Y} $, we obtain 
	\begin{equation}
		I(\rv{X};\rv{Y}) = 1- h_b(\alpha)  \geq C_1.
	\end{equation}
	As we have shown, it is optimal to take the constraint with equality, therefore,
	\begin{equation}
		\alpha = h_b^{-1} (1-C_1).
	\end{equation}

	 Utilizing the fact that $ \mathsf{P}_{\rv{X}\rv{Y}} $ is a \acrshort{dsbs}, let us introduce an auxiliary random variable $ \rv{W} \sim \Ber(\alpha) $, i.e, $ \rv{X} = \rv{Y} + \rv{W} $. Now, lets consider the objective function and try to find an upper bound.
	\begin{align}
		I(\rv{X};\rv{Z}) 
		&= H(\rv{X}) - H(\rv{X}|\rv{Z}) \\
		&= 1 - H(\rv{Y} + \rv{W}|\rv{Z}) \\
		&\eqann{\leq}{a} 1 - h_b(h_b^{-1}(\alpha * H(\rv{Y}|\rv{Z})) ) \\
		&= 1 - h_b(\alpha * h_b^{-1}(1-I(\rv{Y};\rv{Z})) ) \\
		&\leq 1 - h_b(\alpha * h_b^{-1}(1-C_2) ) \\
		&= 1 - h_b(\alpha * \beta)
	\end{align}
	where \eqannref{a} follows from Mrs. Gerber's Lemma \cite{Wyner1973}. Moreover, this bound can be attained by choosing $ \mathsf{P}_{\rv{Z}|\rv{Y}} $ as a \acrshort{bsc} with parameter $ \beta $. Therefore,
	\begin{equation} 
		R^{\text{ob}}(C_1,C_2) = \max_{\mathsf{P}_{\rv{Z}| \rv{Y}}: I(\rv{Y};\rv{Z})\leq C_2} \min_{\mathsf{P}_{\rv{X} \rv{Y}}: I(\rv{X};\rv{Y}) \geq C_1} I(\rv{X};\rv{Z}) = 1 - h_b(\alpha * \beta).
	\end{equation}
	This concludes the proof of the theorem.
\end{proof}





==> sections/continuous_time_channels.tex <==






\begin{figure}
    \centering
    \input{figures/continuous_time_diagram1}
    \caption{Block diagram of Information Bottleneck for Continuous Time Gaussian random processes.}
    \label{fig:comib_continuous_time_diagram1}
\end{figure}


We next consider the case where $\rv{X}(t)$ and $\rv{Y}(t)$ are continuous time Gaussian random processes, i.e.,
\begin{equation*}
    \rv{X}(t) = \rv{Y}(t) + \rv{W}(t),
\end{equation*}
where $\rv{Y}(t)$ is a Gaussian process with power spectral density $S(f) $, and
$\rv{W}(t)$ is an additive Gaussian noise with an arbitrary noise power spectrum $ N(f) $ satisfying $\frac{1}{T} I_T[\rv{X}(t);\rv{Y}(t)] \geq C_T $, where $C = \lim_{T \rightarrow \infty} C_T $ \cite[Ch. 8]{Gallager1968}. We are interested in the following variant of \acrlong{ib} for Gaussian random processes, i.e., we aim to solve the following optimization problem:
\begin{equation}
    \begin{aligned}
    & R_T(C_{T}) =
    && \underset{
    \pmf{\rv{Z}|\rv{Y}}}{\text{maximize}}
    && \frac{1}{T} I_T[\rv{X}(t);\rv{Z}] \\
    &&& \text{subject to}
    && \frac{1}{T} I_T[\rv{Y}(t);\rv{Z}] \leq C_{T},
    \end{aligned}
\end{equation}
and
\begin{equation}
    R(C) = \lim_{T\rightarrow \infty} R_T(C_T).
\end{equation}.

\begin{theorem} \label{theorem:ib_continuous_Gaussian_RP}
The optimal continuous Gaussian \acrshort{ib} rate has the following water-filling form
\begin{equation} \label{eq:ib_continuous_Gaussian_RP_rate}
    R(C_2) = \int \frac{1}{2} \log 
    \left[ \left( 
    1+ \frac{S(f)}{N(f)} \right)
    \frac{\nu-1}{\nu}
    \right]^+
    \mathrm{d}f,
\end{equation}
where the water level $\nu$ is chosen as the solution of the following equation:
\begin{equation} \label{eq:ib_continuous_Gaussian_RP_water_level}
    C_2 = \int \frac{1}{2} \log \left[  \frac{S(f)}{N(f)} (\nu-1)
    \right]^+
    \mathrm{d}f.
\end{equation}
\end{theorem}

\begin{remark}
    Note that this is a new results and we are considering it as a preliminary result to the compound setting addressed in \autoref{subsection:comib_gaussian_processes}.
\end{remark}


==> sections/convexification.tex <==
In this section we will consider convex envelopes of $ R(C_1,C_2) $ and show that it can be tight for some settings.

\subsection{Minimization Problem}
For a fixed $ \mathsf{P}_{\rv{Z}|\rv{Y}} $, we denote by $ f(C_1;\mathsf{P}_{\rv{Z}|\rv{Y}}) $  the output of the inner minimization problem given in \eqref{eq:definition_oblivious_ib}, i.e.,
\begin{equation}
	f(C_1;\mathsf{P}_{\rv{Z}|\rv{Y}}) \triangleq  \min_{\mathsf{P}_{\rv{X} \rv{Y}}: I(\rv{X};\rv{Y}) \geq C_1} I(\rv{X};\rv{Z}).
\end{equation}
This problem is equivalent (it has the same optimal joint \acrshort{pmf} $ \mathsf{P}_{\rv{X}\rv{Y}} $), to
\begin{equation} \label{eq:definition_oblivious_ib_minimization}
	\psi(\eta)  = \psi(\eta;\mathsf{P}_{\rv{Z}|\rv{Y}}) \triangleq  \max_{\mathsf{P}_{\rv{X} \rv{Y}}: H(\rv{Y}|\rv{X}) = \eta} H(\rv{Z}|\rv{X}).
\end{equation}
We denote the upper concave envelope of $ \psi(\eta) $ as $ \varphi(\eta) $. Namely, $ \varphi(\eta) $ is the minimal concave function such that $ \varphi(\eta) \geq \psi(\eta) $.

\begin{remark}
	Note that in general $ \psi(\eta) $ is not concave, but, as was shown in, if the condition $ \sum_{y}
	 \mathsf{P}_{\rv{X}\rv{Y}}(x,y) = \mathsf{P}_{\rv{X}} (x) $ is omitted, then it is a concave function.
\end{remark}

\begin{theorem}
	The supremum of the conditional output entropy rate of a sequence of $ K $ outputs $ \rv{Z}^K $ with respective input $ \rv{X}^K $ over all joint distributions $ \mathsf{P}_{\rv{X}^K\rv{Y}^k} $ and $ K >0 $ is
	\begin{equation}
		\varphi(\eta) = \sup_{K >0 . \mathsf{P}_{\rv{X} \rv{Y}}: \frac{1}{K} H(\rv{Y}^K|\rv{X}^K) = \eta} \frac{1}{K} H(\rv{Z}^K|\rv{X}^K),
	\end{equation}
	namely, the RHS is a concave function of $ \eta $.
\end{theorem}

\begin{proof}
	Since the underlying channels are memoryless, and utilizing the definitions of $ \psi(\cdot) $ and $ \varphi(\cdot) $, we obtain the following list of inequalities:
	\begin{align}
		\frac{1}{K} H(\rv{Z}^K|\rv{X}^K)
		&= \frac{1}{K} \sum_{k=1}^{K} H(\rv{Z}_k|\rv{X}_k) \\
		&\leq \frac{1}{K} \sum_{k=1}^{K} \psi (H(\rv{Y}_k|\rv{X}_k)) \\
		&\leq \frac{1}{K} \sum_{k=1}^{K} \varphi (H(\rv{Y}_k|\rv{X}_k)) \\
		&\leq \varphi \left( \frac{1}{K} \sum_{k=1}^{K}  H(\rv{Y}_k|\rv{X}_k) \right) \\
		&= \varphi \left(\frac{1}{K} H(\rv{Y}^K|\rv{X}^K)\right) \\
		&= \varphi(\eta).
	\end{align}
	If $ \psi(\eta) = \varphi(\eta ) $, then equality achieved for any $  K \geq 1 $. If $ \psi(\eta) < \varphi(\eta ) $, then the point $ (\eta,\varphi(\eta)) $ is a convex combination of two points $ (\eta_1,\psi(\eta_1)) $ and $ (\eta_2,\psi(\eta_2)) $, of the graph of $ \psi(\cdot) $, corresponding to joint probability vectors $ \mathsf{P}_{\rv{X}\rv{Y}}^{(1)} $ and $ \mathsf{P}_{\rv{X}\rv{Y}}^{(2)} $. Namely. there exists $ \lambda \in [0,1] $, s.t.,
	\begin{equation}
		\eta = \lambda \eta_1 + (1-\lambda)\eta_2  \qquad \text{ and } \qquad
		\varphi(\eta) = \lambda \psi(\eta_1) + (1-\lambda) \psi(\eta_2).
	\end{equation}
	If $ \lambda $ is rational, i.e, there exist $ a,b  \in \field{N} $ and $ \lambda = a/b $, take independent $ \{(\rv{X}_i,\rv{Y}_i)\}_{i=1}^b $ of which $ a $ have distribution $  \mathsf{P}_{\rv{X}\rv{Y}}^{(1)} $ and $ b-a $ have distribution $ \mathsf{P}_{\rv{X}\rv{Y}}^{(2)} $, i.e.,
	\begin{equation}
		\mathsf{P}_{\rv{X}^b \rv{Y}^b} (x^b,y^b) = \prod_{i=1}^{a} \mathsf{P}_{\rv{X}\rv{Y}}^{(1)}(x_i,y_i) 
		\cdot
		\prod_{j=a+1}^{b} \mathsf{P}_{\rv{X}\rv{Y}}^{(2)}(x_j,y_j)
	\end{equation}
	we obtain the point $ (\eta,\varphi(\eta)) $, and achieve equality. If $ \lambda $ is irrational, then for any $ 0 < \epsilon < \eta_2 $, we have
	\begin{equation}
		\eta = \lambda_\epsilon \eta_1 + (1-\lambda_\epsilon) (\eta_2 - \epsilon)
	\end{equation}
	with
	\begin{equation}
		\lambda_\epsilon \triangleq \frac{\lambda (\eta_2-\eta_1)-\epsilon}{(\eta_2-\eta_1) - \epsilon}.
	\end{equation}
	Thus,
	\begin{equation}
		\zeta_{\epsilon} = \lambda_\epsilon \psi(\eta_1) + (1-\lambda_\epsilon) \psi(\eta_2 - \epsilon)
	\end{equation}
	is achievable when $ \lambda_\epsilon $ is rational. Taking $ \epsilon \rightarrow 0 $, $ \zeta_{\epsilon} \rightarrow \varphi(\eta) $ and since $ \lambda_\epsilon \rightarrow \lambda $ through an interval, in which rationals are dense, the supremum cannot be less than $ \varphi(\eta) $, completing the proof.
\end{proof}

\begin{corollary}
	Let
	\begin{equation}
		f^{(K)}(C_1;\mathsf{P}_{\rv{Z}^K|\rv{Y}^K}) \triangleq  \min_{\mathsf{P}_{\rv{X}^K \rv{Y}^K}: \frac{1}{K} I(\rv{X}^K;\rv{Y}^K) \geq C_1} \frac{1}{K} I(\rv{X}^K;\rv{Z}^K).
	\end{equation}
	then $ \inf_{K >0} f^{(K)}(C_1;\mathsf{P}_{\rv{Z}^K|\rv{Y}^K}) $  is a convex function of $ C_1 $.
\end{corollary}

\subsection{The Composite Problem}
Consider next the compound setting,
\begin{equation} 
	R^{(K)}(C_1,C_2) = \max_{\mathsf{P}_{\rv{Z}^K| \rv{Y}^K}:  \frac{1}{K}I(\rv{Y}^K;\rv{Z}^K)\leq C_2} \inf_{K >0} f^{(K)}(C_1;\mathsf{P}_{\rv{Z}^K|\rv{Y}^K})
\end{equation}

\begin{proposition}
	$ R^{(K)} (C_1,C_2) $ is convex in $ C_2 $ for fixed $ C_1 $ as a pointwise supremum over an infinite set of convex functions (see \cite[p. 81]{Boyd2014}).
\end{proposition}

\begin{remark}
	For a fixed $ \mathsf{P}_{\rv{X}\rv{Y}} $ the function 
	\begin{equation} 
		R^{\text{ib}}(C) = \max_{\mathsf{P}_{\rv{Z}| \rv{Y}}: I(\rv{Y};\rv{Z})\leq C}  I(\rv{X};\rv{Z}).
	\end{equation}
	is concave in $ C $. This is a known result for the standard \acrshort{ib} problem.
\end{remark}



==> sections/gaussian/comib_continuous_time_channels.tex <==
Equipped with the result of \autoref{theorem:ib_continuous_Gaussian_RP} (continuous time \acrshort{ib}) we next consider the respective compound setting of the problem from the previous section, i.e.,
\begin{equation}
    \begin{aligned}
    & R_T(C_{T}) =
    && \max_{\pmf{\rv{Z}|\rv{Y}}} \min_{\pmf{\rv{X}\rv{Y}}}
    && \frac{1}{T} I_T[\rv{X}(t);\rv{Z}] \\
    &&& \text{subject to}
    && \frac{1}{T} I_T[\rv{Y}(t);\rv{Z}] \leq C_{2T} \\
    &&&&& \frac{1}{T} I_T[\rv{X}(t);\rv{Y}(t)] \geq C_{1T}.
    \end{aligned}
\end{equation}

\begin{theorem} \label{theorem:comib_continuous_gaussian_RP}
    Suppose that $\rv{X}(t)$ and $\rv{W}(t)$ are band-limited random Gaussian processes with one-sided bandwidth $BW$ with unknown power spectral densities $S(f)$ and $N(f)$ respectively.
    We obtain here that it is optimal to take
\begin{equation}
    \frac{S(f)}{N(f)} = 
    \begin{cases}
    S & |f| \leq BW \\
    0 & |f| > BW
    \end{cases},
\end{equation}
where $S$ is the solution to
\begin{equation}
    C_1 = BW \cdot \log \left(1+ S \right),
\end{equation}
and $\nu$ is the solution to 
\begin{equation}
    C_2 = BW \cdot \log S(\nu-1).
\end{equation}
Thus,
\begin{equation}
    R(C_1,C_2) = BW \cdot \log \left[ \frac{1}
    {1-\left(1-2^{-\frac{C_1}{W}} \right)
    \left(1-2^{-\frac{C_2}{W})}
    \right)
    }
    \right].
\end{equation}
\end{theorem}

The above result has the following practical implication. Suppose that you have a continuous time system with an ADC and a compression device. The most robust approach in case there is no information regarding the structure of the observed signal and noise is to assume the input is white and perform a uniform sampling.

==> sections/gaussian/proof_comib_continuous_time_channels.tex <==
Here again we apply the saddle-point optimality property \autoref{lemma:optimality_saddle_point}. 

First direction. Assume 
\begin{equation}
    \frac{S(f)}{N(f)} =
    \begin{cases}
    S & |f| \leq W, \\
    0 & |f| > W.
    \end{cases}
\end{equation}
Thus, from \autoref{theorem:ib_continuous_Gaussian_RP} we have
\begin{equation}
    C_2 = W \log [S(\nu-1)], 
\end{equation}
which implies
\begin{equation}
    \nu^* = 1+ \frac{1}{S} \cdot 2^{\frac{C_2}{W}}.
\end{equation}
Plugging $\nu^*$ in \eqref{eq:ib_continuous_Gaussian_RP_rate} we obtain
\begin{equation}
    R(C_2) = W \log \left[ 
    \frac{1}{1-\frac{S}{1+S} \left( 1-2^{-\frac{C_2}{W}} \right)} \right],
\end{equation}
where $S$ must satisfy the mutual information constraint on $I[\rv{X}(t);\rv{Y}(t)]$, namely,
\begin{equation}
    C_1 = W \log \left( 1+ S \right),
\end{equation}
which indicates
\begin{equation}
    S =  2^{\frac{C_1}{W}} -1 .
\end{equation}
Thus
\begin{equation}
    R(C_1,C_2) \leq - W \log \left[ 
    1- \left(1-2^{-\frac{C_1}{W}} \right) \left(1-2^{-\frac{C_2}{W}} \right)
    \right].
\end{equation}

Opposite direction. Suppose that the channel from $\rv{Y}(t)$ to $\rv{Z}$ is an additive band-limited white Guassian noise channel with $\rv{Y}(t)$ being a Gaussian random process with white power spectral density, i.e.,
\begin{equation}
    \rv{Z}(t) = \gamma \rv{Y}(t) + \sqrt{1-\gamma} \rv{V}(t) = \gamma \left( \rv{X}(t) + \rv{W}(t) \right) + \sqrt{1-\gamma} \rv{V}(t).
\end{equation}
Let $\phi_1(t)$, $\phi_2(t)$ be a complete set of real orthonormal functions over $(0,T)$. We can represent $\rv{X}(t)$ as $\bv{X} = (\rv{X}_1,\rv{X}_2,\dots) ^T$ where
\begin{equation}
    \rv{X}_i = \langle \rv{X},\phi_i \rangle = \int_0^T \rv{X}(t) \phi_i(t) \mathrm{d}t.
\end{equation}
Similarly, we can represent $\rv{Y}(t)$ with $\bv{Y} = (\rv{Y}_1,\rv{Y}_2,\dots )^T$ where:
\begin{align}
    \rv{Y}_i 
    &= \langle \rv{Y},\phi_i \rangle .
\end{align}
Also, we can represent $\rv{Z}(t)$ with $\bv{Z} = (\rv{Z}_1,\rv{Z}_2,\dots )^T$ where:
\begin{align}
    \rv{Z}_i 
    &= \langle \rv{Z},\phi_i \rangle .
\end{align}
Fix $N$ and consider the vectors $ \bv{X} = \rv{X}^N$, $ \bv{Y} = \rv{Y}^N$, $ \bv{Z} = \rv{Z}^N$, which are jointly Gaussian by construction. Furthermore, since $\{\phi_i (t) \}$ is an orthonormal set and $\rv{Y}(t)$ and $\rv{V}(t)$ are white Gaussian processes, the \acrshort{svd} decomposition of $\Sigma_{\bv{Z}}^{-1/2} \Sigma_{\bv{Z}\bv{Y}} \Sigma_{\bv{Y}}^{-1/2} = U_2^T \Gamma V_2 $, has $\Gamma = \gamma I$. Thus, by \autoref{theorem:comib_pf_vector_gaussian}, we have
\begin{equation}
    R_T(C_{1T},C_{2T}) \geq 
    - \frac{N}{2T} \log \left[ 1- \left(1-2^{-\frac{2 T C_1}{N}} \right)
    \left(1-2^{-\frac{2 T C_2}{N}} \right) \right].
\end{equation}
Taking $ N = 2WT$ as in \cite[Thm. 8.2.1]{Gallager1968} (the number of orthonormal functions of duration $T$ and bandwidth $W$), we obtain
\begin{equation}
    R(C_1,C_2) \geq -W \log \left[
    1-
    \left(
    1-2^{-\frac{C_1}{W}}
    \right)\left(1-2^{-\frac{C_2}{W}} \right) 
    \right],
\end{equation}
thus proving the theorem.

Suppose that 
\begin{equation}
    \rv{Z}_i = \gamma \rv{Y}_i + \sqrt{1-\gamma^2} \rv{V}_i, \quad i \in \field{N},
\end{equation}
where $\{\rv{Y}_i\}_{i \geq 1}$ and $\{\rv{V}_i\}_{i \geq 1}$ are Gaussian random processes with zero mean and normalized white spectrum, i.e,
\begin{equation}
    S_{\rv{Y}}(f) = S_{\rv{V}}(f) =
    1 , \quad |f| \leq \frac{1}{2}.
\end{equation}

==> sections/gaussian/proof_ib_continuous_time_channels.tex <==
Consider the problem illustrated in \autoref{fig:comib_continuous_time_diagram1}. Note that $\rv{Y}(t)$ and $\rv{W}(t)$ can be both formed by passing normalized white Gaussian noise through filters with frequency response $\sqrt{S(f)}$ and $\sqrt{N(f)}$, respectively. Let $\tilde{\rv{Y}}(t)$ and $\tilde{\rv{W}}(t)$ be two independent normalized white Gaussian noise processes, an equivalent problem is presented in \autoref{fig:comib_continuous_time_diagram2}. Assuming that $N(f) $ does not vanish at the region of interest (otherwise we may transmit infinitely many bits of information in the respective region),  we can further move the filter with frequency response $\sqrt{N(f)}$ to the output while manipulating the input filter frequency response as shown in \autoref{fig:comib_continuous_time_diagram3}.
This is an equivalent model to the one considered in \cite[Sec. 8.5]{Gallager1968} with $H_1(f) = \sqrt{S(f)}$. In particular, it has an equivalent parallel channel representation illustrated in \autoref{fig:comib_continuous_time_diagram4}, where random variables $ \rv{W}_i $ and $\rv{Y}_i $ are independent normalized Gaussian random variables, namely, $\rv{W}_i \sim \mathcal{N}(0,1)$ and $\rv{Y}_i \sim \mathcal{N} (0,1)$. Furthermore, $\{\lambda_i\}_{i>1} $ can be regarded as the eigenvalues of the filter $K(t,\tau)$ which is defined as
\begin{equation}
    K(t,\tau)
    =
    \begin{cases}
        K_1(t-\tau) & |\tau| \leq T/2 \\
        0 & |\tau| > T/2
    \end{cases},
\end{equation}
with $K_1(t)$ being the impulse response of the filter $ \sqrt{S(f)}/\sqrt{N(f)}$, i.e.,
\begin{equation}
    K_1(t) \triangleq \int \sqrt{\frac{S(f)}{N(f)}} e^{j2\pi f t} \mathrm{d}f.
\end{equation}



\begin{figure}[t]
    \centering
    \input{figures/continuous_time_diagram2}
    \caption{Block diagram of Information Bottleneck for Continuous Time Gaussian random processes. First equivalent representation.}
    \label{fig:comib_continuous_time_diagram2}
\end{figure}

\begin{figure}[b]
    \centering
    \input{figures/continuous_time_diagram3}
    \caption{Block diagram of Information Bottleneck for Continuous Time Gaussian random processes. Second equivalent representation.}
    \label{fig:comib_continuous_time_diagram3}
\end{figure}

\begin{figure}[t]
    \centering
    \input{figures/continuous_time_diagram4}
    \caption{Block diagram of Information Bottleneck for Continuous Time Gaussian random processes. Parallel discrete-time equivalent representation.}
    \label{fig:comib_continuous_time_diagram4}
\end{figure}



Consider a fixed $N$. We are interested in the following maximization problem:
\begin{equation}
    \begin{aligned}
    &\underset{\mathsf{P}_{\rv{Z}|\rv{Y}^N}}{\text{maximize}}
    && I(\rv{U}^N;\rv{Z}) \\
    &\text{subject to} 
    && I(\rv{Y}^N;\rv{Z}) \leq C_2.
    \end{aligned}
\end{equation}

This is exactly the problem solved in \autoref{theorem:ib_jointly_gaussian_vectors} with $d_i = \frac{\sqrt{\lambda_i}}{\sqrt{1+\lambda_i}}$, therefore,
\begin{equation}
    R_T(C_T) = 
    \frac{1}{T}
    \sum_{i=1}^\infty \frac{1}{2} \log 
    \left[
    \frac{(\nu - 1)(1+\lambda_i)}{ \nu }
    \right]^+.
\end{equation}
The water-filling level $\nu$ chosen such that
\begin{equation}
    \frac{1}{T} \sum_{i=1}^\infty \frac{1}{2} \log 
    \left[
    \frac{\frac{\lambda_i}{1+\lambda_i}(\nu - 1)}{1-\frac{\lambda_i}{1+\lambda_i}}
    \right]^+ 
    = \frac{1}{T} 
    \sum_{i=1}^\infty \frac{1}{2} \log 
    \left[
    \lambda_i (\nu-1)
    \right]^+ 
    =
    C_{T}.
\end{equation}


Taking $T \rightarrow \infty$, we obtain
\begin{equation}
    C_2 = \int \frac{1}{2} \log \left[  \frac{S(f)}{N(f)} (\nu-1)
    \right]^+
    \mathrm{d}f,
\end{equation}
and

\begin{equation}
    R(C_2) = \int \frac{1}{2} \log 
    \left[ \left( 
    1+ \frac{S(f)}{N(f)} \right)
    \frac{\nu-1}{\nu}
    \right]^+
    \mathrm{d}f.
\end{equation}

==> sections/high_snr.tex <==
In this section we will consider a regime with $ \eta_1 \in (0,\log 2) $ which can be regarded as a high-\acrshort{snr} regime. Suppose $ \mathsf{P}_{\rv{W}} $ is a negative Hamming \acrshort{pmf} with parameters $ (\beta,n,2) $, therefore,
\begin{equation}
	\mathsf{P}_{\rv{W}} = [\beta \cdot \bv{e}_2 + \bar{\beta} \bv{u}_2 , \bv{0}_{n-2}].
\end{equation}
For an arbitrary input probability vector $ \bv{p} $, the resulting output distribution is given by
\begin{equation}
	[\bv{q}]_i = \left(\beta + \frac{\bar{\beta}}{2}\right) p_i + \frac{\bar{\beta}}{2} p_{i+1}.
\end{equation}
We are interested to find a lower bound on our problem, i.e., solving \eqref{eq:definition_oblib_modulo_lb2}. The respective minimization problem may be reformulated in the following standard form:
\begin{equation}
	\begin{aligned}
		\min_{\bv{p} \in  \field{R}^n} \quad & \sum_{i=1}^n h\left( \left(\beta + \frac{\bar{\beta}}{2}\right) p_i + \frac{\bar{\beta}}{2} p_{i+1}\right) \\
		\textrm{s.t.} \quad & -\sum_{i=1}^n p_i \log p_i = \eta_2 \\
		& \sum_{i=1}^n p_i = 1.
	\end{aligned}
\end{equation}
where $ p_{n+1} \triangleq p_1 $.

Now, consider an arbitrary $ \bv{p} \in \simplex{n} $ satisfying $ h(\bv{p}) = \eta_2 $. Consider a triple of coefficients from $ \bv{p} $, $ (p_{k_1},p_{k_2},p_{k_3}) $, while other coefficients remain fixed. We ask whether $ (p_{k_1},p_{k_2},p_{k_3}) $ is optimal, namely,  is there a different triple satisfying the same respective constraints, but obtains a lower output entropy value. The corresponding local optimization problem takes the following form
\begin{equation}\label{eq:oblib_low_snr_local_optimization}
	\begin{aligned}
		\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & \sum_{\cup \{i: i=k_1,i+1=k_1,i=k_2,i+1=k_2,i=k_3,i+1=k_3\} } h \left( \left(\frac{1+\beta}{2}\right) p_i +\left( \frac{1-\beta}{2}\right) p_{i+1}\right)  \\
		\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i} = \eta_2 + \sum_{i  \in [n] /  \{k_1,k_2,k_3\} }  p_i \log p_i \triangleq c_2\\
		& \sum_{i=1}^3 p_{k_i} = 1 - \sum_{i \in [n]/\{k_1,k_2,k_3\} }p_i \triangleq c_1.
	\end{aligned}
\end{equation}
We denote $ \beta^+ \triangleq (1+\beta)/2 $, $ \beta^- \triangleq (1-\beta)/2 $, $ \gamma_{k} \triangleq \gamma_{k-1} $ and $ \bar{\gamma}_{k} \triangleq \gamma_{k+1} $.

\subsection{Witsenhausen Approach}
Here we apply a directional derivative technique similar to \cite{Witsenhausen1974}. We will need to consider three different configurations for the the triple $ k_1,k_2,k_3 $: the case where they are consecutive; the case where two of them are adjacent; and the case where none of them are adjacent.
\begin{itemize}
	\item In the case $ k_1 < k_1+1 < k_2 < k_2+1< k_3 $, the minimization problem takes the following form:
	\begin{equation}
		\begin{aligned}
			\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & \sum_{i=1}^{3} h\left(  \beta^+ \gamma_{k_i} + \beta^-  p_{k_i} \right) + h\left( \beta^+ p_{k_i} + \beta^-  \bar{\gamma}_{k_i} \right) \\
			\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i} = c_2\\
			& \sum_{i=1}^3 p_{k_i} = c_1.
		\end{aligned}
	\end{equation}
	
	The directional derivative of the objective function is given by
	\begin{align}
		&-\left[\beta^- \log(\beta^+ \gamma_{k_1} + \beta^- p_{k_1}) + \beta^+ \log(\beta^+ p_{k_1} + \beta^- \bar{\gamma}_{k_1}) \right] \mathrm{d} p_{k_1} \\
		&-\left[\beta^- \log(\beta^+ \gamma_{k_2} + \beta^- p_{k_2}) + \beta^+ \log(\beta^+ p_{k_1} + \beta^- \bar{\gamma}_{k_2}) \right] \mathrm{d} p_{k_2} \\
		&-\left[\beta^- \log(\beta^+ \gamma_{k_3} + \beta^- p_{k_3}) + \beta^+ \log(\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}) \right] \mathrm{d} p_{k_3}  \\
		&=- \mathrm{d} p_{k_1} \bigg[\beta^- \log \left(\frac{\beta^+ \gamma_{k_1} + \beta^- p_{k_1}}{\beta^+ \gamma_{k_2} + \beta^- p_{k_2}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_1} + \beta^- \bar{\gamma}_{k_1}}{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}} \right)  \\
		&-\frac{\log p_{k_1} - \log p_{k_2}}{\log p_{k_2} - \log p_{k_1}} \left[
		\beta^- \log \left(\frac{\beta^+ \gamma_{k_2} + \beta^- p_{k_2}}{\beta^+ \gamma_{k_3} + \beta^- p_{k_3}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}}{\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}} \right)
		\right]
		\bigg] .
	\end{align}
	\item If $ k_1 + 1 = k_2 $ and $ k_3  \neq \{k_1-1, k_2+1\}  $, the respective minimization problem becomes:
	\begin{equation}
		\begin{aligned}
			\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & h\left(  \beta^+ \gamma_{k_1} + \beta^-  p_{k_1} \right) + h\left( \beta^+ p_{k_1} + \beta^-  p_{k_2} \right) + h\left( \beta^+ p_{k_2} + \beta^-  \bar{\gamma}_{k_2} \right)  \\
			&+ h\left( \beta^+ \gamma_{k_3} + \beta^-  p_{k_3} \right) +  h\left( \beta^+ p_{k_3} + \beta^-  \bar{\gamma}_{k_3} \right)\\
			\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i}  = c_2\\
			& \sum_{i=1}^3 p_{k_i}  = c_1.
		\end{aligned}
	\end{equation}
	The directional derivative of the objective function is given by
	\begin{align}
		&-\left[\beta^- \log(\beta^+ \gamma_{k_1} + \beta^- p_{k_1}) + \beta^+ \log(\beta^+ p_{k_1} + \beta^- p_{k_2}) \right] \mathrm{d} p_{k_1} \\
		&-\left[\beta^- \log(\beta^+ p_{k_1} + \beta^- p_{k_2}) + \beta^+ \log(\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}) \right] \mathrm{d} p_{k_2} \\
		&-\left[\beta^- \log(\beta^+ \gamma_{k_3} + \beta^- p_{k_3}) + \beta^+ \log(\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}) \right] \mathrm{d} p_{k_3}  \\
		&=- \mathrm{d} p_{k_1} \bigg[\beta^- \log \left(\frac{\beta^+ \gamma_{k_1} + \beta^- p_{k_1}}{\beta^+ p_{k_1} + \beta^- p_{k_2}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}} \right)  \\
		&-\frac{\log p_{k_1} - \log p_{k_2}}{\log p_{k_2} - \log p_{k_1}} \left[
		\beta^- \log \left(\frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ \gamma_{k_3} + \beta^- p_{k_3}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}}{\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}} \right)
		\right]
		\bigg] 
	\end{align}
	\item As for the case $ k_1 + 1 = k_2 = k_3-1 $,  the minimization problem has the following form:
	\begin{equation}
		\begin{aligned}
			\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & h\left(  \beta^+ \gamma_{k_1} + \beta^-  p_{k_1} \right) + h\left( \beta^+ p_{k_1} + \beta^-  p_{k_2} \right) + h\left( \beta^+ p_{k_2} + \beta^-  p_{k_3} \right)  + h\left( \beta^+ p_{k_3} + \beta^-  \bar{\gamma}_{k_3} \right)\\
			\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i}  = c_2\\
			& \sum_{i=1}^3 p_{k_i}  = c_1.
		\end{aligned}
	\end{equation}
	The directional derivative of the objective function is given by
	\begin{align}
		&-\left[\beta^- \log(\beta^+ \gamma_{k_1} + \beta^- p_{k_1}) + \beta^+ \log(\beta^+ p_{k_1} + \beta^- p_{k_2}) \right] \mathrm{d} p_{k_1} \\
		&-\left[\beta^- \log(\beta^+ p_{k_1} + \beta^- p_{k_2}) + \beta^+ \log(\beta^+ p_{k_2} + \beta^- p_{k_3}) \right] \mathrm{d} p_{k_2} \\
		&-\left[\beta^- \log(\beta^+ p_{k_2} + \beta^- p_{k_3}) + \beta^+ \log(\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}) \right] \mathrm{d} p_{k_3}  \\
		&=- \mathrm{d} p_{k_1} \bigg[\beta^- \log \left(\frac{\beta^+ \gamma_{k_1} + \beta^- p_{k_1}}{\beta^+ p_{k_1} + \beta^- p_{k_2}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ p_{k_2} + \beta^- p_{k_3}} \right)  \\
		&-\frac{\log p_{k_1} - \log p_{k_2}}{\log p_{k_2} - \log p_{k_1}} \left[
		\beta^- \log \left(\frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ p_{k_2} + \beta^- p_{k_3}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_2} + \beta^- p_{k_3}}{\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}} \right)
		\right]
		\bigg] .
	\end{align}
\end{itemize}

\subsection{Algorithm}
Now we propose a minimization algorithm.
\begin{enumerate}
	\item Draw a point $ \bv{p} \in \simplex{n} $  that satisfies $ h_n(\bv{p}) = \eta_2 $.  Choose an arbitrary triple $ (p_{k_1},p_{k_2},p_{k_3}) $ from $ \bv{p} $ and consider an arc in $ \simplex{3} $ satisfying $ p_{k_1} + p_{k_2} + p_{k_3} = c_1 $,  and $ \sum_{i=1}^3 p_{k_i} \log p_{k_i} = c_2 $. Parameterize the path along the arc with parameter $ t $, i.e., $ (p_{k_1}(t),p_{k_2}(t),p_{k_3}(t)) $, $ t \in [0,1] $, with $ (p_{k_1}(0),p_{k_2}(0),p_{k_3}(0)) $ being the negative Hamming "distribution" and $ (p_{k_1}(1),p_{k_2}(1),p_{k_3}(1)) $ the positive Hamming "distribution" (since $ c_1\leq 1 $ the triple $ (p_{k_1},p_{k_2},p_{k_3}) $  might not be a proper probability vector summing to one).
	\begin{itemize}
		\item If $ k_1+1=k_2=k_3-1 $, increase $ t $ as long as 
		\begin{multline}
			  \beta^- \log \left(\frac{\beta^+ \gamma_{k_1} + \beta^- p_{k_1}}{\beta^+ p_{k_1} + \beta^- p_{k_2}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ p_{k_2} + \beta^- p_{k_3}} \right)  \\
			  -\frac{\log p_{k_1} - \log p_{k_2}}{\log p_{k_2} - \log p_{k_1}} \left[
			  \beta^- \log \left(\frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ p_{k_2} + \beta^- p_{k_3}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_2} + \beta^- p_{k_3}}{\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}} \right)
			  \right]
		\end{multline}
		is positive. If it is positive for every $ t $ then choose $ t=1 $ and $ (p^*_{k_1},p^*_{k_2},p^*_{k_3}) = (p_{k_1}(1),p_{k_2}(1),p_{k_3}(1)) $.
		\item If $ k_1+1=k_2 $, $ k_3 \notin \{k_1-1,k_2+1\} $ then increase $ t $ as long as 
		\begin{multline}
			\beta^- \log \left(\frac{\beta^+ \gamma_{k_1} + \beta^- p_{k_1}}{\beta^+ p_{k_1} + \beta^- p_{k_2}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}} \right)  \\
			 -\frac{\log p_{k_1} - \log p_{k_2}}{\log p_{k_2} - \log p_{k_1}} \left[
			\beta^- \log \left(\frac{\beta^+ p_{k_1} + \beta^- p_{k_2}}{\beta^+ \gamma_{k_3} + \beta^- p_{k_3}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}}{\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}} \right)
			\right]
		\end{multline}
		is positive. If it is positive for every $ t $ then choose $ t=1 $ and $ (p^*_{k_1},p^*_{k_2},p^*_{k_3}) = (p_{k_1}(1),p_{k_2}(1),p_{k_3}(1)) $.
		\item If $ k_1 < k_1+1 < k_2 < k_2+1< k_3 $ then increase $ t $ as long as 
		\begin{multline}
			\beta^- \log \left(\frac{\beta^+ \gamma_{k_1} + \beta^- p_{k_1}}{\beta^+ \gamma_{k_2} + \beta^- p_{k_2}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_1} + \beta^- \bar{\gamma}_{k_1}}{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}} \right)  \\
			-\frac{\log p_{k_1} - \log p_{k_2}}{\log p_{k_2} - \log p_{k_1}} \left[
			\beta^- \log \left(\frac{\beta^+ \gamma_{k_2} + \beta^- p_{k_2}}{\beta^+ \gamma_{k_3} + \beta^- p_{k_3}} \right)  + \beta^+ \log \left( \frac{\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2}}{\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3}} \right)
			\right]
		\end{multline}
		is positive. If it is positive for every $ t $ then choose $ t=1 $ and $ (p^*_{k_1},p^*_{k_2},p^*_{k_3}) = (p_{k_1}(1),p_{k_2}(1),p_{k_3}(1)) $.
	\end{itemize}
	\item Let $ t^* $ be the optimal parameter on the arc. Replace the triple $ (p_{k_1},p_{k_2},p_{k_3}) $ with $ (p_{k_1}(t^*),p_{k_2}(t^*),p_{k_3}(t^*)) $.
	\item Go to step 1 until a stopping criterion is satisfied: either maximum number of iteration or no further decrease of the output entropy function is possible.
\end{enumerate}

\subsection{Lagrangian Approach}
Next we derive a method to solve \eqref{eq:oblib_low_snr_local_optimization} using Lagrangian multipliers and KKT method.
Similarly here, we are required to consider three different configurations for the the triple $ k_1,k_2,k_3 $: the case where they are consecutive; the case where two of them are adjacent; and the case where none of the are adjacent.
\begin{itemize}
	\item If $ k_1 < k_1+1 < k_2 < k_2+1< k_3 $, the minimization problem obtains the following form:
	\begin{equation}
		\begin{aligned}
			\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & \sum_{i=1}^{3} h\left(  \beta^+ p_{k_i-1} + \beta^-  p_{k_i} \right) + h\left( \beta^+ p_{k_i} + \beta^-  p_{k_i+1} \right) \\
			\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i} =  c_2\\
			& \sum_{i=1}^3 p_{k_i} = c_1.
		\end{aligned}
	\end{equation}
	
	
	The respective Lagrangian takes the form
	\begin{multline}
		L(p_{k_1},p_{k_2},p_{k_3},\lambda ,\mu) \\
		= \sum_{i=1}^{3} h\left(  \beta^+ p_{k_i-1} + \beta^-  p_{k_i} \right) + h\left( \beta^+ p_{k_i} + \beta^-  p_{k_i+1} \right)  + \lambda \left(\sum_{i=1}^3 p_{k_i} \log p_{k_i} + c_2\right) + \mu \left(\sum_{i=1}^3 p_{k_i}  - c_1\right).
	\end{multline}
	Assume that a local optimum of the problem is regular. Then the KKT conditions
	are necessary for a solution, and except for primal and dual feasibility
	state that:
	\begin{itemize}
		\item Stationarity (S): 
		\begin{equation}
			\frac{\partial L}{\partial p_{k_i}}= 
			- \beta^- \log (\beta^+  p_{k_i-1} + \beta^{-} p_{k_i})   - \beta^+ \log (\beta^+  p_{k_i} + \beta^{-} p_{k_i+1}) + \lambda + \lambda \log p_{k_i} + \mu = 0
		\end{equation}
		which is equivalent to
		\begin{equation}
			\frac{\left(\beta^+ \gamma + \beta^- p_{k_j} \right) ^{\beta^-} \left(\beta^+ p_{k_j} + \beta^- \bar{\gamma} \right) ^{\beta^+}}{p_{k_j}^{\lambda}} = \exp(\lambda + \mu)
			, \qquad \forall j \in [3].
		\end{equation}
		Since $(\lambda,\mu)\in\field{R}^2 $ we may replace $ \exp(\lambda + \mu) $ with  $\mu_{1}\triangleq\exp(\lambda + \mu)$. So we obtain 
		\begin{equation} \label{eq:oblib_highsnr_noneighbors_stationarity}
			\frac{\left(\beta^+ \gamma + \beta^- p_{k_j} \right) ^{\beta^-} \left(\beta^+ p_{k_j} + \beta^- \bar{\gamma} \right) ^{\beta^+}}{p_{k_j}^{\lambda}} =\mu_1
			, \qquad \forall j \in [3].
		\end{equation}
		We further denote the LHS of \eqref{eq:oblib_highsnr_noneighbors_stationarity} as $ \varphi(p_{k_j},\lambda, \gamma_{k_j},\bar{\gamma}_{k_j}) $, i.e.,
		\begin{equation} \label{eq:psi_definiition}
			\varphi(p,\lambda ,\gamma , \bar{\gamma}) \triangleq \frac{\left(\beta^+ \gamma + \beta^- p \right) ^{\beta^-} \left(\beta^+ p + \beta^- \bar{\gamma} \right) ^{\beta^+}}{p^{\lambda}} .
		\end{equation}
		\item Complementary slackness (CS): $\sum_{i=1}^{3}p_{k_i}=c_1$, and $\sum_{i=1}^{3}p_{k_i} \log p_{k_i}=c_2$.
	\end{itemize}
	\item The case $ k_1 + 1 = k_2 $ and $ k_3  \neq \{k_1-1, k_2+1\}  $. In such case the minimization problem has the following form.
	\begin{equation}
		\begin{aligned}
			\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & h\left(  \beta^+ \gamma_{k_1} + \beta^-  p_{k_1} \right) 
			+ h\left( \beta^+ p_{k_1} + \beta^-  p_{k_2} \right) 
			+ h\left( \beta^+ p_{k_2} + \beta^-  \bar{\gamma}_{k_2} \right)  \\
			&+ h\left( \beta^+ \gamma{k_3} + \beta^-  p_{k_3} \right) 
			+  h\left( \beta^+ p_{k_3} + \beta^-  \bar{\gamma}_{k_3} \right)\\
			\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i}  = c_2\\
			& \sum_{i=1}^3 p_{k_i}  = c_1.
		\end{aligned}
	\end{equation}
	\begin{itemize}
		\item Stationarity (S): 
		\begin{align}
			\frac{\partial L}{\partial p_{k_1}} &= 
			- \beta^- \log (\beta^+  \gamma_{k_1} + \beta^{-} p_{k_1})   - \beta^+ \log (\beta^+  p_{k_1} + \beta^{-} p_{k_2}) + \lambda + \lambda \log p_{k_1} + \mu = 0 \\
			\frac{\partial L}{\partial p_{k_2}} &= 
			- \beta^- \log (\beta^+  p_{k_1} + \beta^{-} p_{k_2})   - \beta^+ \log (\beta^+  p_{k_2} + \beta^{-} \gamma_{k_2}) + \lambda + \lambda \log p_{k_2} + \mu = 0 \\
			\frac{\partial L}{\partial p_{k_3}} &= 
			- \beta^- \log (\beta^+  \gamma_{k_3} + \beta^{-} p_{k_3})   - \beta^+ \log (\beta^+  p_{k_3} + \beta^{-} \gamma_{k_3}) + \lambda + \lambda \log p_{k_3} + \mu = 0
		\end{align}
		which is equivalent to 
		\begin{equation}
			\frac{\left(\beta^+ \gamma_{k_1} + \beta^- p_{k_1} \right) ^{\beta^-} \left(\beta^+ p_{k_1} + \beta^- p_{k_2} \right) ^{\beta^+}}{p_{k_1}^{\lambda}} = 
			\frac{\left(\beta^+ p_{k_1} + \beta^- p_{k_2} \right) ^{\beta^-} \left(\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2} \right) ^{\beta^+}}{p_{k_2}^{\lambda}}
			=\mu_1
		\end{equation}
		and
		\begin{equation}
			\frac{\left(\beta^+ \gamma_{k_3} + \beta^- p_{k_3} \right) ^{\beta^-} \left(\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3} \right) ^{\beta^+}}{p_{k_3}^{\lambda}} = \mu_1.
		\end{equation}
		\item Complementary slackness (CS): $\sum_{i=1}^{3}p_{k_i}=c_1$, and $\sum_{i=1}^{3}p_{k_i} \log p_{k_i}=c_2$.
	\end{itemize}
	\item In the case $ k_1 + 1 = k_2 = k_3-1 $  the minimization problem takes the following form.
	\begin{equation}
		\begin{aligned}
			\min_{(p_{k_1},p_{k_2},p_{k_3}) \in  \field{R}^3} \quad & h\left(  \beta^+ \gamma_{k_1} + \beta^-  p_{k_1} \right) 
			+ h\left( \beta^+ p_{k_1} + \beta^-  p_{k_2} \right) 
			+ h\left( \beta^+ p_{k_2} + \beta^-  p_{k_3} \right)  
			+ h\left( \beta^+ p_{k_3} + \beta^-  \bar{\gamma}_{k_3} \right)\\
			\textrm{s.t.} \quad & -\sum_{i=1}^3 p_{k_i} \log p_{k_i}  = c_2\\
			& \sum_{i=1}^3 p_{k_i}  = c_1.
		\end{aligned}
	\end{equation}
	\begin{itemize}
		\item Stationarity (S): 
		\begin{align}
			\frac{\partial L}{\partial p_{k_1}} &= 
			- \beta^- \log (\beta^+  \gamma_{k_1} + \beta^{-} p_{k_1})   - \beta^+ \log (\beta^+  p_{k_1} + \beta^{-} p_{k_2}) + \lambda + \lambda \log p_{k_1} + \mu = 0 \\
			\frac{\partial L}{\partial p_{k_2}} &= 
			- \beta^- \log (\beta^+  p_{k_1} + \beta^{-} p_{k_2})   - \beta^+ \log (\beta^+  p_{k_2} + \beta^{-} p_{k_3}) + \lambda + \lambda \log p_{k_2} + \mu = 0 \\
			\frac{\partial L}{\partial p_{k_3}} &= 
			- \beta^- \log (\beta^+  p_{k_2} + \beta^{-} p_{k_3})   - \beta^+ \log (\beta^+  p_{k_3} + \beta^{-} \gamma_{k_3}) + \lambda + \lambda \log p_{k_3} + \mu = 0
		\end{align}
		which is equivalent to 
		\begin{multline}
			\frac{\left(\beta^+ \gamma_{k_1} + \beta^- p_{k_1} \right) ^{\beta^-} \left(\beta^+ p_{k_1} + \beta^- p_{k_2} \right) ^{\beta^+}}{p_{k_1}^{\lambda}} \\
			= 
			\frac{\left(\beta^+ p_{k_1} + \beta^- p_{k_2} \right) ^{\beta^-} \left(\beta^+ p_{k_2} + \beta^- p_{k_3} \right) ^{\beta^+}}{p_{k_2}^{\lambda}} 
			=\frac{\left(\beta^+ p_{k_2} + \beta^- p_{k_3} \right) ^{\beta^-} \left(\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3} \right) ^{\beta^+}}{p_{k_3}^{\lambda}} = \mu_1.
		\end{multline}
		\item Complementary slackness (CS): $\sum_{i=1}^{3}p_{k_i}=c_1$, and $\sum_{i=1}^{3}p_{k_i} \log p_{k_i}=c_2$.
	\end{itemize}
\end{itemize}

\subsection{Algorithm}
Now we propose a minimization algorithm.
\begin{enumerate}
	\item Draw a point $ \bv{p} \in \simplex{n} $  that satisfies $ h_n(\bv{p}) = \eta_2 $.  Choose an arbitrary triple $ (p_{k_1},p_{k_2},p_{k_3}) $ from $ \bv{p} $ and consider an arc in $ \simplex{3} $ satisfying $ p_{k_1} + p_{k_2} + p_{k_3} = c_1 $,  and $ \sum_{i=1}^3 p_{k_i} \log p_{k_i} = c_2 $. Parameterize the path along the arc with parameter $ t $, i.e., $ (p_{k_1}(t),p_{k_2}(t),p_{k_3}(t)) $, $ t \in [0,1] $, , with $ (p_{k_1}(0),p_{k_2}(0),p_{k_3}(0)) $ being the negative Hamming "distribution" and $ (p_{k_1}(1),p_{k_2}(1),p_{k_3}(1)) $ the positive Hamming "distribution" (since $ c_1\leq 1 $ the triple $ (p_{k_1},p_{k_2},p_{k_3}) $  might not be a proper probability vector summing to one).
	\begin{itemize}
		\item If $ k_1+1=k_2=k_3-1 $, then find $ t \in [0,1] $ and $ \lambda \in \field{R} $ that satisfy
		\begin{multline}
			\frac{\left(\beta^+ \gamma_{k_1} + \beta^- p_{k_1}(t) \right) ^{\beta^-} \left(\beta^+ p_{k_1}(t)+ \beta^- p_{k_2}(t) \right) ^{\beta^+}}{p_{k_1}^{\lambda}(t)} \\
			= 
			\frac{\left(\beta^+ p_{k_1} (t)+ \beta^- p_{k_2}(t) \right) ^{\beta^-} \left(\beta^+ p_{k_2} (t)+ \beta^- p_{k_3}(t) \right) ^{\beta^+}}{p_{k_2}^{\lambda}(t)} 
			=\frac{\left(\beta^+ p_{k_2}(t) + \beta^- p_{k_3} (t) \right) ^{\beta^-} \left(\beta^+ p_{k_3} (t)+ \beta^- \bar{\gamma}_{k_3} \right) ^{\beta^+}}{p_{k_3}^{\lambda}(t)} .
		\end{multline}
		\item If $ k_1+1=k_2 $, $ k_3 \notin \{k_1-1,k_2+1\} $ then find $ t \in [0,1] $ and $ \lambda \in \field{R} $ that satisfy
		\begin{multline}
			\frac{\left(\beta^+ \gamma_{k_1} + \beta^- p_{k_1} \right) ^{\beta^-} \left(\beta^+ p_{k_1} + \beta^- p_{k_2} \right) ^{\beta^+}}{p_{k_1}^{\lambda}} \\
			= 
			\frac{\left(\beta^+ p_{k_1} + \beta^- p_{k_2} \right) ^{\beta^-} \left(\beta^+ p_{k_2} + \beta^- \bar{\gamma}_{k_2} \right) ^{\beta^+}}{p_{k_2}^{\lambda}} 
			= \frac{\left(\beta^+ \gamma_{k_3} + \beta^- p_{k_3} \right) ^{\beta^-} \left(\beta^+ p_{k_3} + \beta^- \bar{\gamma}_{k_3} \right) ^{\beta^+}}{p_{k_3}^{\lambda}} 
		\end{multline}
		\item If $ k_1 < k_1+1 < k_2 < k_2+1< k_3 $ then find $ t \in [0,1] $ and $ \lambda \in \field{R} $ that satisfy
		\begin{equation}
			\varphi(p_{k_1}(t),\lambda ,\gamma _{k_1}, \bar{\gamma}_{k_1}) = \varphi(p_{k_2}(t),\lambda ,\gamma _{k_1}, \bar{\gamma}_{k_1}) = \varphi(p_{k_3}(t),\lambda ,\gamma _{k_1}, \bar{\gamma}_{k_1}) .
		\end{equation}
	\end{itemize}
\end{enumerate}


==> sections/main_results.tex <==
In this section we present our main analytical results in this work. We first give a complete characterization of \eqref{eq: oblivious bottleneck additive channels} for a "low-snr" regime of $ \eta_1 $, for the remaining scenarios we provide computable bounds.


\begin{theorem}\label{theorem:oblib_main_result}
	Consider the optimization problem defined in \eqref{eq: oblivious bottleneck additive channels}, and assume that $ \eta_1 \geq \log (n-1) $, then, the optimal $ \mathsf{P}_{\rv{V}} $ and $ \mathsf{P}_{\rv{W}} $ are regular Hamming channel with parameter $ \alpha $ and negative Hamming channel with parameters $ (\beta,n,n) $, where $ \alpha $ is the positive root of 
	\begin{equation}
		\eta_2 + \left(\alpha + \frac{\bar{\alpha}}{n}\right) \log \left(\alpha + \frac{\bar{\alpha}}{n}\right) + \frac{(n-1)\bar{\alpha}}{n} \log 	\frac{\bar\alpha}{n} = 0 .
	\end{equation}
	and $ \beta $ is the negative root of
	\begin{equation}
		\eta_1  + \left(\beta + \frac{\bar{\beta}}{n}\right) \log \left(\beta + \frac{\bar{\beta}}{n}\right) + \frac{(n-1)\bar{\beta}}{n} \log \frac{\bar\beta}{n} = 0.
	\end{equation}
	and
	\begin{equation}
		R(\eta_1,\eta_2) = -\left(\alpha \beta + \frac{\overline{\alpha \beta}}{n}\right) \log \left(\alpha \beta + \frac{\overline{\alpha \beta}}{n}\right) + \frac{(n-1)\overline{\alpha \beta}}{n} \log 	\frac{\overline{\alpha \beta}}{n}
	\end{equation}
\end{theorem}
We postpone the proof of this theorem to \autoref{section:oblib_proof_of_theorem_low_snr}.

Unfortunately, the latter elegant result does not extends for the regime $ \eta_1 \in (0, \log(n-1)) $. Consider the following counterexample. Suppose $ \mathsf{P}_{\rv{W}} $ is a negative Hamming channel with parameters $ (0.46,3,2) $ and take $ \eta_2 = 0.7 $. In such case the positive Hamming point is given by
\begin{equation}
	\bv{p}^{+} = 
	\begin{pmatrix}
		0.8666 \\ 0.0667 \\ 0.0677
	\end{pmatrix}
\end{equation}
which achieves the following output entropy
\begin{equation}
	h(\mat{T} \bv{p}^{+}) = 1.1792.
\end{equation}
But taking
\begin{equation}
	\bv{p}^* = 
	\begin{pmatrix}
		0.857 \\ 0.031 \\ 0.112
	\end{pmatrix}
\end{equation}
gives us
\begin{equation}
	h(\mat{T} \bv{p}^*) = 1.1657 < h(\mat{T} \bv{p}^{+}).
\end{equation}

To further convince ourselves, lets plot the value of the output entropy defined by $ h(\bv{p}) = \eta $ and $ \bv{e}^T \bv{p} = 1 $. The results are shown in \autoref{figure:neghamming3_output_entropy_on_arc}. We observe that the bounds become tighter for small valued of $ \eta_{1} $.

\begin{figure}
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/oblib/neghamming/neghamming3_p2vsp1}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/oblib/neghamming/neghamming3_output_entropy}
		\caption{}
	\end{subfigure}
	\caption{(a) Optimal $ \bv{w} $ for $ \alpha= 0.2 $ vs $ C $. (b) $ R_{T_{\alpha}} (C) $ vs $ C $ for $ \alpha=0.2 $.}
	\label{figure:tito_typewriter_vs_C_alpha_0p2}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/oblib/neghamming/neghamming3_p2vsp1}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/oblib/neghamming/neghamming3_output_entropy}
		\caption{}
	\end{subfigure}
	\caption{(a) Arc on $ \simplex{3} $ satisfying $ h(\bv{p}) = 0.7 $. (b) Output entropy on the arc..}
	\label{figure:neghamming3_output_entropy_on_arc}
\end{figure}

For the regime $ \eta_1 \in (0,\log (n-1)) $ we have only lower and upper bounds on $ R(\eta_1,\eta_2) $. Assume that $ \eta_1 \in (\log(n-2) , \log (n-1)) $, than we have the following result.

\begin{theorem}\label{theorem:oblib_main_result_bounds}
	Consider the regime $ \eta_1 \in (\log(n-2),\log(n-1)) $, then
	\begin{equation}
		R(\eta_1,\eta_2) 
		\leq h  \left(\alpha \beta + \frac{\alpha \bar{\beta}}{n-1} + \frac{\bar{\alpha}}{n} \right) 
		+  (n-2) h\left( \frac{\alpha \bar{\beta}}{n-1} + \frac{\bar{\alpha}}{n} \right) +
		h\left(  \frac{\bar{\alpha}}{n} \right)  .
	\end{equation}
	Suppose $ n=3 $, then we have the following bounds
	\begin{multline}
		(1+\beta)   h_2\left(\frac{1-\alpha}{3}\right) +(1+\beta)  \left(1-\frac{1-\alpha}{3}\right) \log (2) -\beta \eta_2 
		\leq R(\eta_1,\eta_2) \\
		\leq h  \left(\alpha \beta + \frac{\alpha \bar{\beta}}{n-1} + \frac{\bar{\alpha}}{n} \right) 
		+  (n-2) h\left( \frac{\alpha \bar{\beta}}{n-1} + \frac{\bar{\alpha}}{n} \right) +
		h\left(  \frac{\bar{\alpha}}{n} \right)  .
	\end{multline}
	and the difference between the upper and lower bounds are bounded by ???
\end{theorem}
The proof of this theorem is relegated to \autoref{section:oblib_proof_of_main_result_bounds}.

The upper and lower bounds for $ n=3 $, vs $ \eta_2 \in [0, \log (3)] $ are shown in \autoref{figure:oblib_bounds_vs_eta2_n3}.

Follow up question: Assuming $P_{X}$ is uniform, $Y=X+W$, can we
prove that $P_{Z|Y}$ is an additive modulo channel $Z=Y+V$?

\begin{figure}
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/oblib/oblib_bounds_vs_eta2_n3_eta1_0p5}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/oblib/oblib_bounds_vs_eta2_n3_eta1_0p1}
		\caption{}
	\end{subfigure}
	\caption{Bounds (a)  $ \eta_1= 0.5 $  (b) $ \eta_1= 0.1 $ .}
	\label{figure:oblib_bounds_vs_eta2_n3}
\end{figure}

==> sections/modulo_additiveness_Pzgy.tex <==
We assume here that the channel from $ \rv{X} $ to $ \rv{Y} $ is a modulo additive channel and $ \rv{X} $ has a uniform distribution over $[n]$. Therefore, $ \rv{Y} $ is also uniformly distributed over $ [n] $ and the transition matrix from $ \rv{Y} $ to $ \rv{X} $ has a symmetry group of size $ n $, characterized using a set of $ n $ circular permutation matrices $ \left\{ \mat{\Pi}_i \right\}_{i=1}^n $. In particular, let $ T $, be a transition matrix from $ \rv{Y} $ to $ \rv{X} $, then
\begin{equation}
    \Pi_i T = T \Pi_i, \quad \forall i\in \{1,2,\dots,n\}.
\end{equation}
For a fixed $ \pmf{\rv{X}\rv{Y}} $, we aim to describe the solution of the following optimization problem:
\begin{equation} 
    \begin{aligned}
	    & R^{\text{IB}}_{\scaleto{\mathsf{P}_{\rv{X}\rv{Y}}}{4pt}}(C) \triangleq 
	    &&  \underset{\mathsf{P}_{\rv{Z}|\rv{Y}}}{\text{maximize}}
	    &&  I(\rv{X};\rv{Z}) \\
	    &
	    & & \text{subject to}
        & & I(\rv{Y};\rv{\rv{Z}}) \mkern-3mu \leq \mkern-3mu  C.
    \end{aligned}
\end{equation}
But since $\pmf{\rv{X}}$ and $\pmf{\rv{Y}}$ are fixed, we may specialize that problem to the following equivalent minimization problem:
\begin{equation} 
    \begin{aligned}
	    & f^{\text{CEB}}_{\scaleto{\mathsf{P}_{\rv{X}\rv{Y}}}{4pt}}(\eta) \triangleq 
	    &&  \underset{\mathsf{P}_{\rv{Z}|\rv{Y}}}{\text{minimize}}
	    &&  H(\rv{X}|\rv{Z}) \\
	    &
	    & & \text{subject to}
        & & H(\rv{Y}|\rv{\rv{Z}}) \mkern-3mu \geq \mkern-3mu  \eta,
    \end{aligned}
\end{equation}
where $\eta \triangleq \log n - C $.
The latter is exactly the \acrfull{ceb} problem considered in \cite{Witsenhausen1975}. Note that here the optimization includes the cardinality of $ \rv{Z} $. We next focus on the reverse channel from $Z$ to $Y$. Let $ \{ \bv{p}_z \}_{z \in \set{Z}} $ be the columns of the transition probability matrix from $\rv{Z} $ to $ \rv{Y} $, and $ \{ q_z \}_{z \in \set{Z}}  $ be the respective elements of the marginal distribution of $\rv{Z}$. With these definitions we obtain the following optimization problem:
\begin{equation} 
    \begin{aligned}
	    & f^{\text{CEB}}_{\scaleto{T}{4pt}}(\eta) \triangleq 
	    &&  \underset{\{\bv{p}_z,q_z\}_{z\in \set{Z}}}{\text{minimize}}
	    &&  \sum_{z\in \set{Z}} h_n(T\bv{p}_z) q_z \\
	    &
	    & & \text{subject to}
        & & \sum_{z\in \set{Z}} h_n(\bv{p}_z) q_z \mkern-3mu = \mkern-3mu  \eta, \\
        &&&&& \sum_{z\in \set{Z}} \bv{p}_z q_z = \bv{u}.
    \end{aligned}
\end{equation}
Thus, the solution of the problem, is basically a convex combination of various columns of the transition probability matrix that satisfy the average entropy constraint. This problem has a solution (see the arguments in \cite{Witsenhausen1975} for details), and suppose it is given by the set $ \{\bv{p}_z \}_{z \in \set{Z}} $. Let 
\begin{equation}
  \bv{p}^* = \argmin_{\{\bv{p}_z \}_{z \in \set{Z}}} h_n(T\bv{p}_z).  
\end{equation}
Using the definition of $\bv{p}^*$, construct a set of $n$ points in $\simplex{n}$ using the symmetry set of the transition matrix $T$,
\begin{equation}
    \bv{p}^*_{i} \triangleq \Pi _i \bv{p}^* \quad i \in [n].
\end{equation}
Note that due to the symmetry property of $\{ \Pi_i\} _{i=1}^n$ and since entropy function is invariant under permutation we have
\begin{equation}
    h_n(T\bv{p}^*_{i}) = h_n(T \Pi_i \bv{p}^*) = h_n( \Pi_i T \bv{p}^*) = h_n( T \bv{p}^*).
\end{equation}
Furthermore, 
\begin{equation}
    \frac{1}{n} \sum_{i=1}^n \bv{p}_i^* = \frac{1}{n} \sum_{i=1}^n \Pi_i \bv{p}^* = \bv{u}.
\end{equation}
Thus, we have shown, that for $\eta = h_n(\bv{p}^*) $, the solution of the optimization problem is a Modulo Additive channel. 

==> sections/properties_of_covex_functions.tex <==
\begin{lemma}[Slope monotonicity of convex function] \label{lemma:convex_function_slope_monotonicity}
	Suppose $ \phi(t) $ is a convex function, then for every $ t_1 \geq t_2 \geq t_3 $ it holds that
	\begin{equation}
		\frac{\varphi(t_1) - \varphi(t_2)}{t_1-t_2} \geq \frac{\varphi(t_2) - \varphi(t_3)}{t_2-t_3}.
	\end{equation}
\end{lemma}
\begin{proof}
	Since $ \varphi(t) $ is convex, we have for any $ t_1 $, $ t_3 $ and $ \lambda \in [0,1] $,
	\begin{equation} \label{eq:concavity_of_varphi}
		\varphi(\lambda t_1 + \bar{\lambda} t_3) \leq \lambda \varphi(t_1) + \bar{\lambda} \varphi(t_3).
	\end{equation}
	Choosing $ \lambda = \frac{t_2-t_3}{t_1-t_3} $, and plugging it in \eqref{eq:concavity_of_varphi}, we obtain:
	\begin{equation}
		\frac{t_2-t_3}{t_1-t_3} \left[\varphi(t_2) - \varphi(t_1)\right] \leq \frac{t_1-t_2}{t_1-t_3} \left[\varphi(t_3) - \varphi(t_2)\right]
	\end{equation}
	This completes the proof of the lemma.
\end{proof}

==> sections/ternary_alpha.tex <==
For the case $ \alpha $ is arbitrary, and assuming $ \alpha < 1/2 $, we can write the output probability vector from \eqref{eq:neghamming_output_probability_vector} in the following way,
\begin{equation} \label{eq:neghamming_output_probability_vector2}
	\bv{q} =
	\begin{pmatrix}
		q_1 \\ q_2 \\ q_3
	\end{pmatrix}
	\triangleq 
	\mat{T} \bv{p} =
	\alpha 
	\begin{pmatrix}
		p_1 + p_2 \\
		p_2 + p_3 \\
		p_3 + p_1
	\end{pmatrix}
	+(1-2\alpha) \bv{p}	
	=
	2\alpha \frac{1}{2} 
	\begin{pmatrix}
		1-p_3 \\
		1-p_1 \\
		1-p_2
	\end{pmatrix}
	+(1-2\alpha) \bv{p}	
\end{equation}
Using concavity of the entropy function, we have
\begin{align}
	h(\mat{T} \bv{p}) 
	&=2\alpha h \left(
	 \frac{1}{2} 
	\begin{pmatrix}
		1-p_3 \\
		1-p_1 \\
		1-p_2
	\end{pmatrix}
	+(1-2\alpha) \bv{p}	
	\right) \\
	&\geq
	2\alpha h\left( \frac{1}{2} 
	\begin{pmatrix}
		1-p_3 \\
		1-p_1 \\
		1-p_2
	\end{pmatrix}
	\right)
	+(1-2\alpha) h(\bv{p}) \\
	&\geq
	2\alpha h\left( \frac{1}{2} 
	\begin{pmatrix}
		1-p_3 \\
		1-p_1 \\
		1-p_2
	\end{pmatrix}
	\right)
	+(1-2\alpha)  \eta
\end{align}
Thus,
\begin{align}
	\min_{\bv{p} \colon  h(\bv{p})\geq\eta} h(\mat{T} \bv{p}) 
	&\geq \min_{\bv{p} \colon  h(\bv{p})\geq\eta}
	\left\{
	2\alpha h\left( \frac{1}{2} 
	\begin{pmatrix}
		1-p_3 \\
		1-p_1 \\
		1-p_2
	\end{pmatrix}
	\right)
	+(1-2\alpha)  \eta
	\right\} \\
	&\geq 2\alpha \min_{\bv{p} \colon  h(\bv{p})\geq\eta}
	\left\{
	 h\left( \frac{1}{2} 
	\begin{pmatrix}
		1-p_3 \\
		1-p_1 \\
		1-p_2
	\end{pmatrix}
	\right)
	\right\}
	+(1-2\alpha)  \eta
\end{align}
where the solution for inner minimization follows from the special case of $ \alpha = 0.5 $.

==> sections/ternary_alpha0p5.tex <==
We begin the discussion we a special case of $ \alpha = 0.5 $, i.e,
\begin{equation}
	\mat{T} =
	\begin{pmatrix}
		\frac{1}{2} &  \frac{1}{2} & 0 \\
		0 & \frac{1}{2} & \frac{1}{2} \\
		\frac{1}{2} & 0 & \frac{1}{2}
	\end{pmatrix}.
\end{equation}
Thus,
\begin{equation}
	\mat{T} \bv{p} = 
	\begin{pmatrix}
		\frac{p_1+p_2}{2} \\
		\frac{p_2+p_3}{2} \\
		\frac{p_3+p_1}{2} 
	\end{pmatrix}
	= 
	\begin{pmatrix}
		\frac{1-p_3}{2} \\
		\frac{1-p_1}{2} \\
		\frac{1-p_2}{2} 
	\end{pmatrix},
\end{equation}


==> sections/tito.tex <==
The general \acrfull{tito} Circulant Matrix is defined as follows:
\begin{equation} \label{eq:tito_transition_matrix}
	T = 
	\begin{pmatrix}
		1-\alpha-\beta & \alpha & \beta \\
		\beta & 1-\alpha-\beta  & \alpha \\
		\alpha & \beta & 1-\alpha - \beta
	\end{pmatrix}.
\end{equation}
The respective symmetry group consists of the following matrices:
\begin{equation}
	\mat{G}_1 =
	\begin{pmatrix}
		1 & 0 & 0 \\
		0 & 1 & 0 \\
		0 & 0 & 1
	\end{pmatrix}
	=\mat{\Pi}_1,
	\qquad
	\mat{G}_2 =
	\begin{pmatrix}		
		0 & 1 & 0 \\
		0 & 0 & 1\\
		1 & 0 & 0 
	\end{pmatrix}
	=\mat{\Pi}_2,
	\qquad
	\mat{G}_3 =
	\begin{pmatrix}		
		0 & 0 & 1\\
		1 & 0 & 0 \\
		0 & 1 & 0 
	\end{pmatrix}
	=\mat{\Pi}_3.
\end{equation}
Note that $ \mat{G}_1 \mat{T} = \mat{T} \mat{\Pi}_1 $, and
\begin{align}
	\mat{G}_2 \mat{T} 
	&= 
	\begin{pmatrix}		
		0 & 1 & 0 \\
		0 & 0 & 1\\
		1 & 0 & 0 
	\end{pmatrix}
	\begin{pmatrix}
		1-\alpha-\beta & \alpha & \beta \\
		\beta & 1-\alpha-\beta  & \alpha \\
		\alpha & \beta & 1-\alpha - \beta
	\end{pmatrix}
	\\
	&= 
	\begin{pmatrix}
		\beta & 1-\alpha -\beta & \alpha \\
		\alpha & \beta & 1-\alpha - \beta \\
		1-\alpha-\beta & \alpha & \beta 
	\end{pmatrix}	 \\
	&=
	\begin{pmatrix}
		1-\alpha-\beta & \alpha & \beta \\
		\beta & 1-\alpha-\beta  & \alpha \\
		\alpha & \beta & 1-\alpha - \beta
	\end{pmatrix}
	\begin{pmatrix}		
		0 & 1 & 0 \\
		0 & 0 & 1\\
		1 & 0 & 0 
	\end{pmatrix}\\
	&= T \Pi_2.
\end{align}
Similarly, $ \mat{G}_3 \mat{T}_3 = \mat{T}_3 \mat{\Pi}_3 $.

Now, fix $ \lambda \in (0,1) $ and let $ \bv{p}_\lambda $ be the minimizer of $ \phi(\bv{p},\lambda) $, .i.e.,
\begin{equation}
	\bv{p}_\lambda \triangleq \argmin_{\bv{p} \in \simplex{3}} \phi(\bv{p},\lambda).
\end{equation}
$ \bv{p}_\lambda $ can be found by denoting $ \bv{p} \triangleq  (p,r,1-p-r)^T $, and find the pair $ (p_\lambda,r_\lambda) $ that solve the following list of equations:
\begin{align}
	\frac{\partial \phi}{\partial p} &= 0 \\
	\frac{\partial \phi}{\partial r} &= 0.
\end{align}
Since $ \lambda $ is fixed, we compute the respective constraint as follows
\begin{equation}
	C_\lambda = \log 3 -  h_3(\bv{p}_{\lambda}).
\end{equation}
The optimal rate in this case would be
\begin{equation}
	R(C_\lambda) = \log 3 - h_3(\mat{T} \bv{p}_{\lambda}).
\end{equation}

We can further ask if there are values of  $ C $ such that $ R(C) $ can be achieved with $ \rv{Z}  $ taking two points. The following corollary states the opposite.
\begin{corollary}
	The minimum cardinality of $ \rv{Z} $ that achieves $ R(C) $ is exactly 3 for $ C \neq 0 $.
\end{corollary}
\begin{proof}
	In general, for every $ \bv{p}_1 = \bv{p}_\lambda = (p_\lambda,r_\lambda,1-p_\lambda-r_\lambda)^T $ that minimizes $ \phi(\bv{p},\lambda) $, there exists
	\begin{equation}
		\bv{p}_2= \Pi_2 \bv{p}_1 = 
		\begin{pmatrix}
			r_\lambda \\ 1-p_\lambda-r_\lambda \\ p_\lambda
		\end{pmatrix}
		\qquad
		\bv{p}_3= \Pi_3 \bv{p}_1 = 
		\begin{pmatrix}
			1-p_\lambda-r_\lambda \\ p_\lambda \\ r_\lambda.
		\end{pmatrix}
	\end{equation}
	Assume that $ |\set{Z}|=2 $, therefore either $ \bv{p}_1 = \bv{p}_2 $ or $ \bv{p}_1 = \bv{p}_3 $ or $ \bv{p}_2 = \bv{p}_3 $. Any of this conditions imply that $ \bv{p}_1 = \bv{p}_2 = \bv{p}_3 = \bv{u}_3 $, and $ |\set{W}| = 1 $. This implies that $ |\set{\rv{Z}}|\neq 2 $ and if $ |\set{Z}| = 1 $, than $ C = \log 3 - h(\bv{u}_3) = 0 $.
\end{proof}

Next, we evaluate $ \bv{p}_\lambda $ and $ R(C_\lambda) $ for some specific choices of $ T $, i.e., $ (\alpha,\beta) $.

\begin{figure}[b]
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_hamming_Pw_vs_alpha_C_1}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_hamming_R_vs_alpha_C_1}
		\caption{}
	\end{subfigure}
	\caption{(a) Optimal $ \bv{w} $ for $ C = 1 $ vs $ \alpha $. (b) $ R_{T_{\alpha}} (C) $ vs $ \alpha $ for $ C=1 $.}
	\label{figure:tito_hamming_vs_alpha_C_1}
\end{figure}

\subsubsection{The Supper-Symmetric \acrshort{tito}}
First, consider a specific, super-symmetric case where $ \alpha = \beta $ in \eqref{eq:tito_transition_matrix}. This is also known as  the third order Hamming channel with parameter $ \alpha $ \cite[Sec. IV.E]{Witsenhausen1975}. For this, super-symmetric formulation we have the following characterization of the channel $ \mathsf{P}_{\rv{Y}|\rv{Z}} $.
\begin{proposition} \label{proposition:tito3_hamming}
	The optimal channel from $ \rv{Y} $ to $ \rv{Z} $ is also a super-symmetric channel with parameter $ \delta $, where
	$ \delta = g_3^{-1}(C)  $, with $ g_3(x) \triangleq \log 3 +2x\log x + (1-2x) \log(1-2x) $.
\end{proposition}
\begin{proof}
	For $ \alpha = \beta $,
	\begin{equation}
		\mat{T} \bv{p} = 
		\begin{pmatrix}
			(1-2\alpha)  p + \alpha r + \alpha(1-p-r) \\
			\alpha p+(1-2\alpha)  r  + \alpha(1-p-r) \\
			\alpha p+\alpha  r  + (1-2\alpha)(1-p-r)
		\end{pmatrix}
		=
		\begin{pmatrix}
			(1-3\alpha)  p  + \alpha \\
			(1-3\alpha)  r  + \alpha \\
			(1-3\alpha)(1-p-r) + \alpha
		\end{pmatrix}
	\end{equation}
	Therefore,
	\begin{align}
		\nabla_{\bv{p}} \phi(\bv{p},\lambda)
		&= 
		\begin{pmatrix}
			\frac{\partial \phi}{\partial p} \\
			\frac{\partial \phi}{\partial r}
		\end{pmatrix} \\
		&=
		\begin{pmatrix}
			(1-3\alpha) \log \frac{(1-3\alpha)(1-p-r) + \alpha}{(1-3\alpha)  p + \alpha} + \lambda \log \frac{p}{1-p-r} \\
			(1-3\alpha) \log \frac{(1-3\alpha)(1-p-r) + \alpha}{(1-3\alpha)  r + \alpha} + \lambda \log \frac{r}{1-p-r}
		\end{pmatrix}
	\end{align}
	The local minimum condition implies that $ \nabla_{\bv{p}} \phi(\bv{p},\lambda) = \bv{0} $, therefore,
	\begin{equation}
		\lambda \log \frac{p}{r} + (1-3\alpha) \log \frac{(1-3\alpha)r+\alpha}{(1-3\alpha)p+\alpha} = 0.
	\end{equation}
	Thus, the minimum point satisfies $ \bv{p}_1= \bv{p}_\lambda = (p_\lambda,p_\lambda,1-2p_{\lambda}) $. Since $ \bv{p}_2 = \mat{\Pi}_2 \bv{p}_{\lambda} $ and $ \bv{p}_3 = \mat{\Pi}_3 \bv{p}_{\lambda} $ are also minimal points of $ \phi(\bv{p},\lambda) $, the transition matrix from $ \rv{Z} $ to $ \rv{Y} $ which columns are the vectors $ \bv{p}_1 $, $ \bv{p}_2 $ and $ \bv{p}_3 $, is also a super-symmetric transition matrix. Moreover, for the Hamming setting, $ p_\lambda $ can be easily computed via the following procedure.
	\begin{align}
		C &= H(\rv{Y}) -   H(\rv{Y}|\rv{Z})\\
		& =\log(3) - h_3(\bv{p}_\lambda) \\
		&= \log(3) +p_\lambda \log p_\lambda + p_\lambda \log p_\lambda+(1-2 p_\lambda) \log (1-2p_\lambda) \\
		&= \log 3  +2p_\lambda \log p_\lambda + (1-2 p_\lambda) \log (1-2p_\lambda) \\
		&\triangleq g_3(p_\lambda)
	\end{align}
	Thus, $ p_\lambda = g_3^{-1}(C) $.
\end{proof}

We further verify \autoref{proposition:tito3_hamming} via numerical simulations. \autoref{figure:tito_hamming_vs_alpha_C_1} shows the probability vector $ \rv{W} $ and $ R_{T_\alpha}(C) $ for various values of $ \alpha $. We observe that the numerical optimization agrees with theoretic arguments in \autoref{proposition:tito3_hamming}. 

Since $ \rv{W} $ is independent of the choice of $ \alpha $, we further freeze $ \alpha = 0.5 $ and compare it with respect to the value of $ C $. The results are shown in \autoref{figure:tito_hamming_vs_C_alpha_0p5}. 



\begin{figure}
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_hamming_Pw_vs_C_alpha_0p5}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_hamming_R_vs_C_alpha_0p5}
		\caption{}
	\end{subfigure}
	\caption{(a) Optimal $ \bv{w} $ for $ \alpha = 0.5 $ vs $ C $. (b) $ R_{T_{\alpha}} (C) $ vs $ C $ for $ \alpha=0.5 $.}
	\label{figure:tito_hamming_vs_C_alpha_0p5}
\end{figure}


Are there other  channels that their Information Bottleneck function can be fully characterized? In the following section we consider  a yet another channel defined by a single parameter.

\subsubsection{The Noisy Typewriter \acrshort{tito}}
Here we consider the case where $ \beta = 0 $ in \eqref{eq:tito_transition_matrix}. This is also known as  the noisy typewriter channel with parameter $ \alpha $. Unfortunately, for this formulation we don't have a simple characterization of the test-channel from $ \rv{Z} $ to $ \rv{Y} $. For $ \beta = 0 $, the transition matrix \eqref{eq:tito_transition_matrix} is given by:
	\begin{equation}
		\mat{T} \bv{p} = 
		\begin{pmatrix}
			(1-\alpha)  p + \alpha r  \\
			(1-\alpha)  r  + \alpha(1-p-r) \\
			\alpha p+ (1-\alpha)(1-p-r)
		\end{pmatrix}
		=
		\begin{pmatrix}
			(1-\alpha)  p  + \alpha r \\
			(1-2\alpha)  r  + \alpha(1-p) \\
			(1-\alpha)(1-r) -(1-2\alpha) p
		\end{pmatrix}.
	\end{equation}
	Therefore,
	\begin{align}
		\nabla_{\bv{p}} \phi(\bv{p},\lambda)
		&= 
		\begin{pmatrix}
			\frac{\partial \phi}{\partial p} \\
			\frac{\partial \phi}{\partial r}
		\end{pmatrix} \\
		&=
		\begin{pmatrix}
			(1-2\alpha) \log \left( \bar{\alpha} \left( 1-p-r \right) + \alpha p \right) + \alpha \log (\alpha \bar{p}+ (1-2\alpha)r) - \bar{\alpha} \log (\bar{\alpha} p +\alpha r)
			+ \lambda \log \frac{p}{1-p-r} \\
			\bar{\alpha} \log \left( \bar{\alpha} \left( 1-p-r \right) + \alpha p \right) - (1-2\alpha) \log (\alpha \bar{p}+ (1-2\alpha)r) - \alpha \log (\bar{\alpha} p +\alpha r) + \lambda \log \frac{r}{1-p-r}
		\end{pmatrix}
	\end{align}
	The local minimum condition implies that $ \nabla_{\bv{p}} \phi(\bv{p},\lambda) = \bv{0} $. Our initial conjecture was that the optimal test-channel here from $ \rv{Z} $ to $ \rv{Y} $ would be also noisy typewriter channel, but as you may observe,  choosing $ p+r=1 $  will not nullify the gradient.
	
	To further convince the reader, we find the optimal test-channel using numerical optimization methods. The result for various values of $ \alpha $ is shown in \autoref{figure:tito_typewriter_vs_alpha_C_0p8}. As can be observed, the optimal test-channel from $ \rv{Z} $ to $ \rv{Y} $ does depend on $ \alpha $. 
	
	We further freeze $ \alpha = 0.2 $ and plot the optimal test-channels for various values of $ C $ as seen in \autoref{figure:tito_typewriter_vs_C_alpha_0p2}. Our only observation is that the optimal test-channel is not noisy-typewriter,  however, one of the elements of $ P_{\rv{W}} $ rapidly tends to zero (red curve in \autoref{figure:tito_typewriter_vs_C_alpha_0p2} (b)).


\begin{figure}
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_typewriter_Pw_vs_alpha_C_0p8}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_typewriter_R_vs_alpha_C_0p8}
		\caption{}
	\end{subfigure}
	\caption{(a) Optimal $ \bv{w} $ for $ C= 0.8 $ vs $ C $. (b) $ R_{T_{\alpha}} (C) $ vs $ \alpha $ for $ C=0.8 $.}
	\label{figure:tito_typewriter_vs_alpha_C_0p8}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_typewriter_Pw_vs_C_alpha_0p2}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[t]{0.49\textwidth}
		\input{../figures/titoIB/tito_typewriter_R_vs_C_alpha_0p2}
		\caption{}
	\end{subfigure}
	\caption{(a) Optimal $ \bv{w} $ for $ \alpha= 0.2 $ vs $ C $. (b) $ R_{T_{\alpha}} (C) $ vs $ C $ for $ \alpha=0.2 $.}
	\label{figure:tito_typewriter_vs_C_alpha_0p2}
\end{figure}




\subsection{The oblivious symmetric bottleneck with $ m=3 $.}
In this section we solve numerically the optimization problem defined in \eqref{eq:definition_sym_oblivious_ib} for $ m=3 $. \autoref{figure:tito_maxmin_iXZ_T_vs_Pw_C_1} shows $ \min_{\mathsf{P}_{\rv{W}}: H(\rv{W})= \log_2(3) - C_1} I(\rv{X};\rv{Z}) $ for various values of $ P_{\rv{V}} $ that satisfy $ H(\rv{V}) = \log_2(3)-C_2 $. We observe that for any choice of $ P_{\rv{V}} $ the minimizer of $ I(\rv{X};\rv{Z}) $ is a noisy-typewriter channel. The optimal $ \mathsf{P}_{\rv{W}} $ and $ \mathsf{P}_{\rv{V}} $ versus  $ C_1 = C_2 = C $ are plotted in \autoref{figure:tito_maxmin_iXZ_T_vs_C}. Note the bifurcation phenomena for $ \mathsf{P}_{\rv{W}} $ when the entropy of $ \rv{W} $ crosses $ H(\rv{W}) = 1 $. We observe that the optimal $ \mathsf{P}_{\rv{W}} $ is the noisy typewriter for $ H(\rv{W}) <1 $, while for $ H(\rv{W}) >1 $ it is a Hamming channel. On the other hand, the optimal $ \mathsf{P}_{\rv{V}} $ is a Hamming channel for any $ C $.

\begin{figure}
	\centering
	\input{../figures/titoIB/tito_maxmin_iXZ_T_vs_Pw_C_1}
	\caption{Evaluation of $ \min I(\rv{X};\rv{Z}) $ and the respective $ P_{\rv{W}} $ that achieves the minimum for various values of $ P_{\rv{V}} $ for $ C_1=C_2=1 $ .}
	\label{figure:tito_maxmin_iXZ_T_vs_Pw_C_1}
\end{figure}

\begin{figure}
	\centering
	\input{../figures/titoIB/tito_maxmin_iXZ_T_vs_C}
	\caption{Evaluation of $ R(C,C) $ and the respective optimal $ \mathsf{P}_{\rv{W}} $ and $ \mathsf{P}_{\rv{V}} $ for various values of  $ C_1=C_2=C $ .}
	\label{figure:tito_maxmin_iXZ_T_vs_C}
\end{figure}


==> sections/total_variation_proof.tex <==
\begin{proof}
Since the total variation satisfies a data-processing theorem, it
holds for any $P_{V}\in\Delta_{n}$ and $P_{W}$ so that $d_{TV}(P_{W},P_{W}^{(0)})\leq\delta$
that
\[
d_{TV}(P_{W}*P_{V},P_{W}^{(0)}*P_{V})\leq d_{TV}(P_{W},P_{W}^{(0)})\leq\delta.
\]
Hence,
\[
\max_{P_{V}\colon H(P_{V})\geq\eta_{2}}\max_{P_{W}\colon d_{TV}(P_{W},P_{W}^{(0)})\leq\delta}d_{TV}(P_{W}*P_{V},P_{W}^{(0)}*P_{V})\leq\delta.
\]
By {[}Zhang 2007, Audenaert 2007{]}, since both $P_{W}*P_{V},P_{W}^{(0)}*P_{V}\in\Delta_{n}$
we obtain
\[
\max_{P_{V}\colon H(P_{V})\geq\eta_{2}}\max_{P_{W}\colon d_{TV}(P_{W},P_{W}^{(0)})\leq\delta}\left|H(P_{W}*P_{V})-H(P_{W}^{(0)}*P_{V})\right|\leq\omega(\delta,n).
\]
Thus, 
\begin{align*}
R(\delta,\eta_{2}) & \leq\min_{P_{V}\colon H(P_{V})\geq\eta_{2}}\max_{P_{W}\colon d_{TV}(P_{W},P_{W}^{(0)})\leq\delta}H(P_{W}^{(0)}*P_{V})+\omega(\delta,n)\\
 & =\min_{P_{V}\colon H(P_{V})\geq\eta_{2}}H(P_{W}^{(0)}*P_{V})+\omega(\delta,n),
\end{align*}
and an analogous lower bound similarly holds. 
\end{proof}


\begin{proof}
To prove the lower bound, note that by the minimax inequality 
\[
R(\eta_{1},\eta_{2})\geq\max_{P_{W}\colon d_{TV}(P_{W},P_{W}^{(0)})\leq\delta}\min_{H(P_{V})\geq\eta_{2}}H(P_{W}*P_{V})
\]
and so any arbitrary choice of $P_{W}$ with $d_{TV}(P_{W},P_{W}^{(0)})\leq\delta$
leads to a valid lower bound. Fix $P_{W}$ and denote for brevity
$T\equiv T(P_{W})$. Then, the lower bound is given by $R(\eta_{1},\eta_{2})\geq g_{T}(\eta_{2})$,
where 
\[
g_{T}(\eta)=\min_{\bv p\in\Delta_{n}\colon H(\bv p)\geq\eta}H(T\bv p)
\]
is Witsenhausen's function from {[}44{]}. Let $p^{*}$ the minimizer
of $g_{T}(\eta)$. It then holds
\begin{align*}
g_{T}(\eta) & \overset{(a)}{\geq}\min_{\bv p\in\Delta_{n}\colon d_{TV}(\bv p,\bv u)\leq d_{TV}(\bv p^{*},\bv u)}H(T\bv p)\\
 & \overset{(b)}{\geq}\min_{\bv p\in\Delta_{n}\colon d_{TV}(T\bv p,T\bv u)\leq\theta(T)\cdot d_{TV}(\bv p^{*},\bv u)}H(T\bv p)\\
 & \overset{(c)}{\geq}\min_{\bv q\in\Delta_{n}\colon d_{TV}(\bv q,\bv u)\leq\theta(T)\cdot d_{TV}(\bv p^{*},\bv u)}H(\bv q)\\
 & \overset{(d)}{\geq}\min_{\bv q\in\Delta_{n}\colon d_{TV}(\bv q,\bv u)\leq\theta(T)\cdot D(\eta)}H(\bv q)\\
 & =\Gamma\left(\theta(T)\cdot D(\eta)\right),
\end{align*}
where $(a)$ follows since $p^{*}$ is optimal for $g_{T}(\eta)$,
$(b)$ follows from the definition of $\theta(T)$, $(c)$ follows
by setting $\bv q=T\bv p$ and relaxing the constraint that $\bv q=T\bv p$,
and $(d)$ follows since $H(p^{*})\geq\eta$, so that 
\[
d_{TV}(\bv p^{*},\bv u)\leq\max_{\bv p\in\Delta_{n}\colon H(\bv p)\geq\eta}d_{TV}(\bv p,\bv u)=D(\eta)
\]
where the last equality holds for $\eta\in[0,\log n]$ by the definition
of $D(\eta)$ is the inverse of $\Gamma(\delta)$. This lower bound
on $g_{T}(\eta)$ then completes the proof of the lower bound for
$R(\eta_{2})$. 

To prove the upper bound, choose an arbitrary $P_{V}$ with $H(P_{V})=\eta_{2}$,
and let $T\equiv T(P_{V})$ be the corresponding channel matrix. Then,
\begin{align*}
R(\delta,\eta_{2}) & \leq\max_{\bv p\in\Delta_{n}\colon d_{TV}(\bv p,\bv p^{(0)})\leq\delta}H(T\bv p)\\
 & \overset{(a)}{\leq}\max_{\bv p\in\Delta_{n}\colon d_{TV}(T\bv p,T\bv p^{(0)})\leq\theta(T)\cdot\delta}H(T\bv p)\\
 & \overset{(b)}{\leq}\max_{\bv q\in\Delta_{n}\colon d_{TV}(\bv q,T\bv p^{(0)})\leq\theta(T)\cdot\delta}H(q)\\
 & =\Phi\left(\theta(T)\cdot\delta;T\bv p^{(0)}\right).
\end{align*}
where $(a)$ follows from the definition of $\theta(T)$ and $(b)$
follows by setting $\bv q=T\bv p$ and relaxing the constraint that
$\bv q=T\bv p$
\end{proof}

==> sections/wasserstein_sinkhorn.tex <==
Denote by $\langle \cdot, \cdot \rangle$ the Frobenius dot-product. For every two probability vectors $\bv{p}, \bv{q} \in \simplex{n} $ we write $U(\bv{p},\bv{q})$ as the transport polytope of $\bv{p}$ and $\bv{q}$, namely the polyhedral set of $n \times. n$ matrices,
\begin{equation}
    U(\bv{p},\bv{q}) \triangleq \left\{
    P \in \field{R}^{n \times n}_{+} \colon P \bv{e} = \bv{p}, P^T \bv{e} = \bv{q}
    \right\}
\end{equation}
Further, the following convex set is defined
\begin{equation}
    U_{\alpha}(\bv{p},\bv{q}) =
    \left\{
    P \in U(\bv{p},\bv{q}) \colon
    D(P||\bv{p}\bv{q}^T) \leq \alpha
    \right\}
\end{equation}
Let $M$ be a metric matrix, namely.
\begin{equation}
    \set{M}
    = 
    \left\{
    M \in \field{R}^{n \times n}
    \right\}
\end{equation}
Sinkhorn distance is defined as
\begin{equation}
    d_{M,\alpha} (\bv{p},\bv{q}) \triangleq \min_{P \in U_{\alpha}(\bv{p},\bv{q})} \langle P, M \rangle .
\end{equation}

In this section we consider the following optimization problem.
\begin{equation}
    R(\delta_1,\delta_2) =
    \max_{f_{\rv{Z}|\rv{Y}} \colon }
    \min_{f_{\rv{X}\rv{Y}} \colon   }
    I(\rv{X};\rv{Z})
\end{equation}
